Efficient Robust Optimal Transport with Application to Multi-Label Classification

Optimal transport (OT) is a powerful geometric tool for comparing two distributions and has been employed in various machine learning applications. In this work, we propose a novel OT formulation that takes feature correlations into account while learning the transport plan between two distributions. We model the feature-feature relationship via a symmetric positive semi-definite Mahalanobis metric in the OT cost function. For a certain class of regularizers on the metric, we show that the optimization strategy can be considerably simplified by exploiting the problem structure. For high-dimensional data, we additionally propose suitable low-dimensional modeling of the Mahalanobis metric. Overall, we view the resulting optimization problem as a non-linear OT problem, which we solve using the Frank-Wolfe algorithm. Empirical results on the discriminative learning setting, such as tag prediction and multi-class classification, illustrate the good performance of our approach.

==> main_camera_ready.tex <==
\begin{abstract}
Optimal transport (OT) is a powerful geometric tool for comparing two distributions and has been employed in various machine learning applications. In this work, we propose a novel OT formulation that takes feature correlations into account while learning the transport plan between two distributions. We model the feature-feature relationship via a symmetric positive semi-definite Mahalanobis metric in the OT cost function. For a certain class of regularizers on the metric, we show that the optimization strategy can be considerably simplified by exploiting the problem structure. For high-dimensional data, we additionally propose suitable low-dimensional modeling of the Mahalanobis metric. Overall, we view the resulting optimization problem as a non-linear OT problem, which we solve using the Frank-Wolfe algorithm. Empirical results on the discriminative learning setting, such as tag prediction and multi-class classification, illustrate the good performance of our approach. 




%The problem of robust optimal transport (OT) aims at recovering the best transport plan with respect to the worst possible cost function. In this work, we study novel robust OT formulations where the cost function is parameterized by a symmetric positive semi-definite Mahalanobis metric. In particular, we study several different regularizations on the Mahalanobis metric -- element-wise $p$-norm, KL-divergence, and doubly-stochastic constraint -- and show that the resulting optimization formulations can be considerably simplified by exploiting the problem structure. For large-scale applications, we additionally propose a suitable low-dimensional decomposition of the Mahalanobis metric for the studied robust OT problems. Overall, we view the robust OT (min-max) optimization problems as non-linear OT (minimization) problems, which we solve using a Frank-Wolfe algorithm. We discuss the use of robust OT distance as a loss function in multi-class/multi-label classification problems. Empirical results on several real-world tag prediction and multi-class datasets show the benefit of our modeling approach. 
\end{abstract}
%For several class of regularizations on the metric, e.g.,  element-wise $p$-norm, KL-divergence, or doubly-stochastic constraint, we show that the optimization of the proposed robust OT problem may be considerably simplified by dropping the positive semi-definite constraint on the metric (but still obtaining a globally optimal solution). 

\section{Introduction}\label{sec:intro}
Optimal transport~\cite{peyre19a} has become a popular tool in diverse machine learning applications such as domain adaptation~\cite{courty17b,nath20a}, natural language processing~\cite{mjaw20b}, %melis18a
computer vision~\cite{rubner00}, and prototype selection~\cite{gurumoorthy21a}, to name a few. The optimal transport (OT) metric between two probability measures, also known as the Wasserstein distance or the earth mover's distance (EMD), defines a geometry over the space of probability measures~\cite{villani09a} and evaluates the minimal amount of work required to transform one measure into another with respect to a {given} ground cost function (also termed as the ground metric or simply the cost function). Due to its desirable metric properties, the Wasserstein distance has also been popularly employed as a loss function in generative and discriminative model training~\cite{frogner15a,genevay18a}. %arjovsky17a

The ground cost function may be viewed as a user-defined parameter in the OT optimization problem. Hence, the effectiveness of an OT distance depends upon the suitability of the (chosen) cost function. Recent works have explored learning the latter by maximizing the OT distance over a set of ground cost functions~\cite{paty19a,paty20a,dhouib20a}. From a dual perspective, this may also be viewed as an instance of robust optimization,  %~\cite{bental09a,bertsimas11a} 
where the transport plan is learned with respect to an adversarially cost function. 
%Works such as~\cite{paty19a,dhouib20a} parameterize the cost function with a Schatten norm regularized Mahalanobis metric to learn a OT distance robust to high dimensional (noisy) data. 
A bottleneck in computing the robust OT distances is the high computational complexity~\cite{paty19a,dhouib20a}, which inhibit their usage as a loss function in large-scale learning applications. 

In this work, we explore OT distances that take feature correlations into account within the given input space. Specifically, we parameterize the cost function with a sparse Mahalanobis metric to learn OT distances robust to  spurious feature correlations present in the data. It should be noted that Mahalanobis metric is a symmetric positive semi-definite matrix and an additional sparsity-inducing constraint/regularization on it may further complicate the optimization problem, potentially leading to a high computational complexity for learning it. In this regard, our main contributions are the following.
\begin{itemize}
\item We discuss three families of sparsity-inducing regularizers for the Mahalanobis metric parameterized cost function:  entry-wise $p$-norm for $p\in(1,2]$, KL-divergence based regularization, and the doubly-stochastic regularization. We show that for those regularizers enforcement of the symmetric positive semi-definite constraint is {\it not} needed as the problem structure {implicitly} learns a symmetric positive semi-definite matrix at optimality. The implications are two fold: a lower computational cost of computing the proposed robust OT distance and a simpler optimization methodology. 
\item To further reduce the computational burden of the proposed robust OT distance computation, we propose a novel $r$-dimensional modeling of the Mahalanobis metric for the studied robust OT problems, resulting in an even lower per-iteration computational cost, where $r \ll d$. The parameter $r$ provides an effective trade-off between computational efficiency and accuracy. 
\item We discuss how to use the robust distance as a loss in discriminative learning settings such as multi-class and multi-label classification problems. Empirically, we observe that computing the proposed robust OT distance is at least {\it $45$ times faster} than existing Mahalanobis metric parameterized robust OT distances \cite{paty19a,dhouib20a} and also obtains better generalization performance as a loss function in discriminative settings. 
\end{itemize}

The proofs and additional experimental results are in our extended draft \cite{jawanpuria20a}.

% The outline of the paper is as follows. Section~\ref{sec:related} presents a brief overview of the relevant OT literature. Section \ref{sec:formulations} discusses the proposed formulations. In Section~\ref{sec:optimization}, we discuss the optimization methodology. 
% %A novel modeling of the metric is discussed in Section \ref{sec:low_dimensional_metric_decomposition}. We formulate the robust OT distance problem as a non-linear OT (minimization) problem in $\gamma$. In Section \ref{sec:algorithms}, this interpretation allows to develop a Frank-Wolfe algorithm. 
% The setup of using the robust OT distance in learning problems is detailed in Section \ref{sec:ROTloss}. In Section \ref{sec:experiments}, we present the empirical results.  

% We begin by briefly discussing relevant optimal transport literature in the next section.

\section{Background and related work}\label{sec:related}
% Given two probability measures $\mu_1$ and $\mu_2$ over metric spaces $\calS$ and $\calT$, respectively, the optimal transport problem due to \cite{kantorovich42a} aims at finding a transport plan $\gamma$ as a solution to the following problem:
% \begin{equation}\label{eqn:optimal-transport}
%     {\rm W}_c(\mu_1,\mu_2) = \inf_{\gamma\in\Pi(\mu_1,\mu_2)} \int_{\calS\times\calT} c(\bs,\bt) d\gamma(\bs,\bt),
% \end{equation}
% where $\Pi(\mu_1,\mu_2)$ is the set of joint distributions with marginals $\mu_1$ and $\mu_2$ and $c:\calS \times \calT \rightarrow \R_{+}:(\bs,\bt)\rightarrow c(\bs,\bt)$ represents the transportation cost function. In several real-world applications, the distributions $\mu_1$ and $\mu_2$ are not available; instead samples from them are given. 
Let $\{\bs_i\}_{i=1}^m\in\R^{d}$ and $\{\bt_j\}_{j=1}^n\in\R^d$ represent iid samples from the source and the target distributions, $\mu_1$ and $\mu_2$, respectively. The empirical estimates of $\mu_1$ and $\mu_2$ supported on the given samples may be defined as 
\begin{equation}
    \hat{\mu}_1\coloneqq\sum_{i=1}^m \bp_i\delta_{\bs_i},\;\;\;\;\;  \hat{\mu}_2\coloneqq\sum_{j=1}^n \bq_j\delta_{\bt_j}.
\end{equation}
Here,  $\delta$ is the delta function and $\bp\in\Delta_m,\bq\in\Delta_n$ are the probability vectors, with $\Delta_d\coloneqq\{\bx\in\R^{d}|\bx\geq\bzero;\bx^\top\bone=1\}$. 
The optimal transport problem due to \cite{kantorovich42a} aims at finding a transport plan $\gamma$ as a solution to the following problem:
\begin{equation}\label{eqn:optimal-transport-discrete}
    {\rm W}_c(\bp,\bq) = \min_{\gamma\in\Pi(\bp,\bq)} \inner{\gamma,\bC},
\end{equation}
where $\bC$ is the $m\times n$ ground cost matrix with $\bC_{ij}=c(\bs_i,\bt_j)$ and $\Pi(\bp,\bq)=\{\gamma\in\R^{m\times n}|\gamma\geq\bzero;\gamma\bone=\bp;\gamma^\top\bone=\bq\}$. The function $c:\R^d \times \R^d \rightarrow \R_{+}:(\bs,\bt)\rightarrow c(\bs,\bt)$ represents the transportation cost function and $\Pi(\bp,\bq)$ is the set of joint distributions with marginals $\hat{\mu}_1$ and $\hat{\mu}_2$. 
% Let $\{\bs_i\}_{i=1}^m\in\R^{d}$ and $\{\bt_j\}_{j=1}^n\in\R^d$ represent $m$ and $n$ iid samples from $\mu_1$ and $\mu_2$, respectively. Then, empirical estimates of $\mu_1$ and $\mu_2$ supported on the given samples, defined as \begin{equation}
%     \hat{\mu}_1\coloneqq\sum_{i=1}^m \bp_i\delta_{\bs_i},\;\;\;\;\;  \hat{\mu}_2\coloneqq\sum_{j=1}^n \bq_j\delta_{\bt_j},
% \end{equation}
% can be employed for computing the OT distance. Here,  $\delta$ is the delta function and $\bp\in\Delta_m$ and $\bq\in\Delta_n$ are the probability vectors, with $\Delta_d\coloneqq\{\bx\in\R^{d}|\bx\geq\bzero;\bx^\top\bone=1\}$. In this setting, the OT problem (\ref{eqn:optimal-transport}) may be rewritten as:
% \begin{equation}\label{eqn:optimal-transport-discrete}
%     {\rm W}_c(\bp,\bq) = \min_{\gamma\in\Pi(\bp,\bq)} \inner{\gamma,\bC},
% \end{equation}
% where $\bC$ is the $m\times n$ ground cost matrix with $\bC_{ij}=c(\bs_i,\bt_j)$ and $\Pi(\bp,\bq)=\{\gamma\in\R^{m\times n}|\gamma\geq\bzero;\gamma\bone=\bp;\gamma^\top\bone=\bq\}$. 
We obtain the popular $2$-Wasserstein distance by setting the cost function as the squared Euclidean function, i.e.,  $c(\bs,\bt)=\norm{\bs-\bt}^2$ when $\bs,\bt\in\R^d$. The $2$-Wasserstein distance can equivalently be reformulated as follows \cite{paty19a}:
\begin{equation}\label{eqn:W22distance}
    {{\rm W}}_2^2(\bp,\bq) = \minop_{\gamma\in\Pi(\bp,\bq)} \inner{\bV_\gamma,\bI},
\end{equation}
where $\bV_\gamma=\sum_{ij} (\bs_i-\bt_j)(\bs_i-\bt_j)^\top \gamma_{ij}$ is the weighted second-order moment of all source-target displacements. 
%where $\bV_\gamma\coloneqq\int_{\calS\times\calT} (\bs-\bt)(\bs-\bt)^\top d\gamma(\bs,\bt)$ and $\bI$ is the identity matrix. In discrete OT setting, when the source and the target distributions are represented by their samples,  $\{\bs_i\}_{i=1}^m\in\R^{d}$ and $\{\bt_j\}_{j=1}^n\in\R^d$, respectively, the expression for $\bV_\gamma$ is:
%\begin{equation}\label{eqn:vgamma}
%    \bV_\gamma=\sum_{ij} (\bs_i-\bt_j)(\bs_i-\bt_j)^\top \gamma_{ij}.
%\end{equation}
% Hence $\bV_\gamma$ may also be viewed as a weighted second-order moment of all source-target displacements. 
%It should be noted that $\bV_\gamma$ is the second-order moment matrix of the displacements associated with a transport plan, i.e., for source and target distribution's samples $\{\bs_i\}_{i=1}^m\in\R^{d}$ and $\{\bt_j\}_{j=1}^n\in\R^d$, respectively, $\bV_\gamma=\sum_{ij} (\bs_i-\bt_j)(\bs_i-\bt_j)^\top \gamma_{ij}$. Hence, the proposed regularization on the metric $\bM$ learns appropriate weights to the individual components of $\bV_\gamma$. In contrast, the ${{\rm W}}_2^2$ distance, defined in (\ref{eqn:W22distance}), has $\bM=\bI$, which enforces the first-order displacements to be uncorrelated and have unit variance. This may be a strong assumption in real-word applications.


% The optimal transport between discrete probability measures $\mu_1$ and $\mu_2$ may be formulated as the following optimization problem \cite{kantorovich42a}: 
% \begin{equation}\label{eqn:optimal-transport}
% {\rm W}_c(\mu_1,\mu_2) = \min_{\gamma\in\Pi(\mu_1,\mu_2)} \inner{\gamma,\bC},
% \end{equation}
% where $\bC\in\R_{+}^{m\times n}$ is a ground cost matrix, $\mu_1\in\Delta_m$, $\mu_2\in\Delta_n$, $\Delta_m\coloneqq\{\bw\R^{m}:\bw\geq\bzero;\bw^\top=1\}$, and $\Pi(\mu_1,\mu_2)$ is the set of joint probability distribution with marginals $\mu_1$ and $\mu_2$, i.e., $\Pi(\mu_1,\mu_2)=\{\gamma\in\R^{m\times n}:\gamma\geq \bzero;\gamma \bone=\mu_1;\gamma^\top\bone=\mu_2\}$. 

% between the source distribution's samples  $\bX=\{\bx_i\}_{i=1}^m\in\R^{d\times m}$ and the target distribution's samples $\bY=\{\by_i\}_{i=1}^n\in\R^{d\times n}$, the $(i,j)$-th entry of $\bC$ is $c(\bx_i,\by_j)$, $c(\bx,\by)$ is the given ground cost function, $\mu_1$ and $\mu_2$ are the given discrete source and target distributions, respectively, and $\Pi(\mu_1,\mu_2)$ is the set of feasible joint transportation plan: $\Pi(\mu_1,\mu_2)=\{\gamma\in\R^{m\times n}:\gamma\geq \bzero;\gamma \bone=\mu_1;\gamma^\top\bone=\mu_2\}$. 
% The special case of $c(\bx,\by)=\norm{\bx-\by}^2$ (squared Euclidean distance) is popularly denoted by ${{\rm W}}_2^2$ (the $2$-Wasserstein distance) and can be reformulated as follows \cite{paty19a}: 
% %$ {{\rm W}}_2^2(\mu_1,\mu_2) = \min_{\gamma\in\Pi(\mu_1,\mu_2)}\ \inner{\bV_\gamma,\bI}$, 
% \begin{equation}\label{eqn:W22distance}
%     {{\rm W}}_2^2(\mu_1,\mu_2) = \minop_{\gamma\in\Pi(\mu_1,\mu_2)}\ \inner{\bV_\gamma,\bI},\\
%     %&=& \minop_{\gamma\in\Pi(\mu_1,\mu_2)} \trace(\bV_\gamma),
% \end{equation}
% where $\bV_\gamma=\sum_{ij} (\bx_i-\by_j)(\bx_i-\by_j)^\top \gamma_{ij}$ and $\bI$ is the identity matrix. 


%\cite{paty19a} proposed a subspace robust variant of the Wasserstein distance that considers the maximal distance between two probability measures when they are projected on a lower dimensional subspace. 
%More generally, 



%\subsection*{Robust optimal transport} 

Recent works \cite{paty19a,kolouri19a} %deshpande19a 
have studied the \textit{minimax} robust variants of the Wasserstein distance that aim at maximizing the OT distance in a projected low-dimensional space. 
%From a duality perspective, these variants may also be viewed as instances of robust OT distance as they learn transport plan corresponding to worst possible ground cost function.  
%Such OT distances are typically modeled as \commentPJ{max-min/min-max} optimization problems and may be viewed as instances of the robust OT distance. 
%In general, the robust OT distance aims at maximizing the minimal transport cost over a set of ground cost functions.
Subspace Robust Wasserstein (SRW) distance~\cite{paty19a} is a robust variant of the ${\rm W}_2^2$ distance, defined as follows: 
%Paty and Cuturi~\cite{paty19a} propose a robust variant of the ${\rm W}_2^2$ distance, termed as the Subspace Robust Wasserstein (SRW) distance, as follows: 
%${{\rm SRW}}_k^2(\mu_1,\mu_2) = \max_{\bM\in\calM}\min_{\gamma\in\Pi(\mu_1,\mu_2)}\ \inner{\bV_\gamma,\bM}$, 
\begin{equation}\label{eqn:SRW1}
%%\begin{array}{lll}
    {{\rm SRW}}_k^2(\bp,\bq) = \minop_{\gamma\in\Pi(\bp,\bq)}\maxop_{\bM\in\calM}\ \inner{\bV_\gamma,\bM},
%    %&=&\minop_{\gamma\in\Pi(\mu_1,\mu_2)} \sum\limits_{i=1}^k \lambda_i(\bV_\gamma),
%%\end{array}
\end{equation}
where the domain $\calM$ is defined as $\calM=\{\bM:\bzero\preceq\bM\preceq\bI {\rm \ and \ } \trace(\bM)=k\}$. 
It should be noted that $\inner{\bV_\gamma,\bM}=\int_{\calS\times\calT} c_\bM(\bs,\bt) d\gamma(\bs,\bt)$, where $c_{\bM}(\bs,\bt)=(\bs-\bt)^\top\bM(\bs-\bt)$ is a cost function parameterized by a Mahalanobis metric (symmetric positive semi-definite matrix) $\bM$ of size $d\times d$. 
%It should be noted that $\inner{\bV_\gamma,\bM}=\sum_{i,j}\gamma_{ij}c_{\bM}(\bx_i,\by_j)$, where $c_{\bM}(\bx,\by)=(\bx-\by)^\top\bM(\bx-\by)$ is a Mahalanobis metric parameterized cost function. 
Similarly, Dhouib~et~al.~\cite{dhouib20a} proposed a variant of robust OT distance (\ref{eqn:SRW1}), but with the domain $\calM$ defined as $\calM=\{\bM:\bM\succeq\bzero {\rm \ and\ } \norm{\bM}_{*p}=1\}$, where $\norm{\cdot}_{*p}$ denotes the Schatten $p$-norm regularizer, i.e., $\norm{\bM}_{*p}\coloneqq(\sum_i \sigma_i(\bM)^p)^\frac{1}{p}$. Here, $\sigma_i(\bM)$ denotes the $i$-th largest eigenvalue of $\bM$. 


Both \cite{paty19a,dhouib20a} pose their Mahalanobis metric parameterized robust OT problems as optimization problems over the metric $\bM$. This usually involves satisfying/enforcing the positive semi-definite (PSD) constraint at every iteration, which requires eigendecomposition operations having $O(d^3)$ computational cost. In this context, Dhouib~et~al.~\cite{dhouib20a} have remarked in their work that ``\textit{...PSD constraints increase considerably the computational burden of any optimization problem, yet they are necessary for the obtained cost function to be a true metric}''. 
In their formulation, \cite{dhouib20a} needs to explicitly enforce the PSD constraint (e.g., via eigendecomposition) for all Schatten $p$-norm regularizers except for $p=2$.
 




%All proofs and additional experimental details are supplied as supplementary material.

%\commentPJ{We can give outline of the paper here and also write about all proofs in the supplementary material.}


















%When $\CC$ is a convex set, robust OT distance may also be modeled via a min-max objective which has the following interpretations: recover the best transport plan with respect to the worst possible ground cost function \cite{dhouib20a}.  
%Robust OT problems have been explored for robustness to noise in high dimensional data \cite{paty19a}, for submodular cost functions. 
%Computing them typically requires solving a a min-max (or a max-min) optimization problem.




% The main contributions of this work are as follows:
% \begin{itemize}
%     \item we propose novel robust OT formulations where the cost function is parameterized by the Mahalanobis metric $\bM\succeq\bzero$. For the proposed families of regularizers on $\bM$, we show that the problem may be solved by dropping the positive semi-definiteness constraint on metric $\bM$ ($\bM\succeq\bzero$) as the resulting optimal solution $\bM^{*}$ satisfies $\bM^{*}\succeq\bzero$. This considerably simplifies our optimization methodology. The proposed family of regularizers on the Mahalanobis metric $\bM$ include entry-wise $p$-norm for $p\in(1,2]$, KL-divergence based regularization, and the doubly stochastic regularization. 
%     \item we develop two approaches for solving the proposed robust OT formulations. The first is a Frank-Wolfe algorithm which requires regularization on the transport plan \cite{cuturi13a} for efficiency. Our second approach employs the Riemannian optimization framework and does not require additional regularization on the transport plan. We propose efficient first- and second-order Riemannian algorithms for the robust OT problems. 
%     \item \commentPJ{Empirical contributions}
% \end{itemize}

% We study robust optimal transport problems of the form:
% \begin{equation}\label{eqn:RKP}
% {\rm RKP}(\Pi,\CC) = \max_{c\in\CC}\min_{\gamma\in\Pi}  \sum\limits_{i,j}\gamma_{ij}c(\bx_i,\by_j),
% \end{equation}
% where $c(\bx,\by)$ is the cost of moving $\bx$ to $\by$ (drawn from distributions $\mu_1$ and $\mu_2$, respectively). Overall, (\ref{eqn:RKP}) aims at learning a cost function, which maximizes the minimium Wasserstein distance between a given pair of distributions. In this work, we study efficient formulations and algorithms for (\ref{eqn:RKP}) when $\CC$ is a convex set. 








% \subsection{Background}
% The optimal transport (OT) problem may be formulated as:
% \begin{equation}\label{eqn:optimal-transport}
% \gamma^{*} \coloneqq \argmin_{\gamma\in\Pi(\mu_1,\mu_2)} \inner{\gamma,\bC}_F,
% \end{equation}
% where $\bC$ is the given cost matrix. The special case of employing the squared Euclidean distance as the cost, popularly denoted by ${{\rm W}}_2^2$ ($2$-Wasserstein distance), is as follows: 
% \begin{equation}\label{eqn:W22distance}
% %\begin{array}{lll}
%     {{\rm W}}_2^2(\mu_1,\mu_2) = \minop_{\gamma\in\Pi(\mu_1,\mu_2)}\ \inner{\bV_\gamma,\bI},\\
%     %&=& \minop_{\gamma\in\Pi(\mu_1,\mu_2)} \trace(\bV_\gamma),
% %\end{array}
% \end{equation}
% where $\bV_\gamma=\sum_{ij} (\bx_i-\by_j)(\bx_i-\by_j)^\top \gamma_{ij}$ and $\bI$ is the identity matrix. 
% \cite{paty19a} propose a robust variant of the $W_2^2$ distance, termed as the Subspace Robust Wasserstein (SRW) distance, as follows:
% \begin{equation}\label{eqn:SRW1}
% %\begin{array}{lll}
%     {{\rm SRW}}_k^2(\mu_1,\mu_2) = \maxop_{\bM\in\calM} \minop_{\gamma\in\Pi(\mu_1,\mu_2)}\ \inner{\bV_\gamma,\bM},\\
%     %&=&\minop_{\gamma\in\Pi(\mu_1,\mu_2)} \sum\limits_{i=1}^k \lambda_i(\bV_\gamma),
% %\end{array}
% \end{equation}
% where the domain $\calM$ is defined as $\calM=\{\bM:\bzero\preceq\bM\preceq\bI; \trace(\bM)=k\}$. 
% It should be noted that $\inner{\bV_\gamma,\bM}=\sum_{i,j}\gamma_{ij}(\bx_i-\by_j)^\top\bM(\bx_i-\by_j)$. 
% Thus, ${{\rm SRW}}_k^2$ learns a worst-case OT cost function  $c_{\bM}(\bx,\by)=(\bx-\by)^\top\bM(\bx-\by)$, which is parameterized by a Mahalanobis metric. 

%The trace regularization in (\ref{eqn:SRW1}) encourages $\bM$ to be of low-rank for $k<d$. It is evident that the SRW distance is an instance of the robust Kantorovich problem (\ref{eqn:RKP}). 
% \begin{equation}\label{eqn:RKP}
% {\rm RKP}(\Pi,\CC) = \min_{\gamma\in\Pi} \max_{c\in\CC} \sum\limits_{i,j}\gamma_{ij}c(\bx_i,\by_j),
% \end{equation}
% where $c(\bx,\by)$ is the cost of moving $\bx$ to $\by$ (drawn from distributions $\mu_1$ and $\mu_2$, respectively). Overall, (\ref{eqn:RKP}) aims at learning a transport plan $\gamma^{*}$ which is robust to the choice of a cost function $c\in\CC$ (best worst achievable transportation cost). 

% Recently, \cite{dhouib20a} study the above form of Mahalanobis metric parameterized cost functions in the robust OT setting, but with the domain $\calM$ defined as $\calM=\{\bM:\bM\succeq\bzero; \norm{\bM}_{*p}=1\}$, where $\norm{\cdot}_{*p}$ denotes the Schatten $p$-norm regularizer, i.e., $\norm{\bM}_{*p}\coloneqq(\sum_i \sigma_i(\bM)^p)^\frac{1}{p}$. Here,   $\sigma_i(\bM)$ denotes the $i$-th largest eigenvalue of $\bM$. 
% They show that this family of regularization include, as special cases, the $W_2^2$ distance with $p=\infty$ (spectral norm) and the $S_1^2$ distance with $p=1$ (trace norm). 

%It should be noted that $p=1$ Schatten norm (the nuclear/trace norm) regularizes the sum of eigenvalues whereas $p=\infty$ Schatten norm (the spectral norm) regularizes the maximum eigenvalue. 


%$\CC_1=\{c^\bM: (\bx,\by)\mapsto (\bx-\by)^\top\bM(\bx-\by);\bM\succeq\bzero,\norm{\bM}_p\leq1\},$
%They show that ${\rm RKP}(\Pi,\CC)=W_2^2(\mu_1,\mu_2)$ with $p=\infty$ and ${\rm RKP}(\Pi,\CC)$ also simplifies to SRW distance \cite{paty19a} with truncated Schatten $p$-norm. The special case of $p=2$ is also discussed in some detail. However, their main contribution is to propose a cutting-set algorithm for solving the general ${\rm RKP}(\Pi,\CC)$ in the discrete case and $\CC$ is an arbitrary convex set of cost matrices with entries $\bC_{ij}=c(\bx_i,\by_j)$.  

%Both \cite{paty19a,dhouib20a} pose their Mahalanobis metric parameterized robust optimal transport problems as an optimization over metric $\bM$. This involves satisfying the positive semi-definite constraint, which typically requires costly eigendecomposition operation of a $d\times d$ matrix in each step. Overall, \cite{paty19a} propose  projected super-gradient and Frank-Wolfe methods to compute the SRW distance (\ref{eqn:SRW1}). \cite{dhouib20a}, on the other hand, propose a cutting-set based method \cite{mutapcic09} to optimize over Schatten $p$-norm regularized Mahalanobis metric. 

%Most existing works solve instances of the robust Kantorovich problem (RKP) (\ref{eqn:RKP}) as an optimization problem over the cost function. \cite{paty19a} solve the max-min problem in (\ref{eqn:SRW1}) via the projected super-gradient and Frank-Wolfe algorithms. While solving the max-min problem, the gradient computation requires solving the inner minimization problem (over $\gamma$), which is an unregularized OT problem, which may be made efficient by regularizing the OT problem \cite{cuturi13a}. \cite{dhouib20a} propose a cutting-set method to solve (\ref{eqn:RKP}) in convex setting. 
%They remark that unlike the robust OT algorithms in \cite{paty19a}, the cutting-set method may also work on non-differentiable robust OT problems. 

%{\color{red} Existing works have studied problem (\ref{eqn:MahalanobisRobustOT}) with the domain $\calM$ defined as $\calM=\{\bM:\bM\succeq\bzero; \norm{\bM}_{*p} \leq 1\}$ \cite{dhouib20a} or $\calM=\{\bM:\bzero\preceq\bM\preceq\bI; \trace(\bM)=k\}$ \cite{paty19a}. They solve the max-min formulation where the outer problem involves positive semi-definite constraints, which typically involves costly eigendecomposition operation of $d\times d$ matrix.}

%It should be noted that the SRW distance is a tight convex relaxation of the (non-convex and non-smooth) projection robust Wasserstein (PRW) distance. \cite{lin20a} propose to directly solve for PRW distance in the Riemannian optimization framework. 








\section{Novel formulations for robust OT}\label{sec:formulations}
We consider a general formulation of Mahalanobis metric parameterized robust optimal transport problem as follows:
%We now discuss the propose novel formulations of the Mahalanobis metric parameterized robust optimal transport problem, which we rewrite as
\begin{equation}\label{eqn:MahalanobisRobustOT}
    {\rm W}_{\rm ROT}(\bp,\bq)\coloneqq\minop_{\gamma\in\Pi(\bp,\bq)}\ f(\gamma),
\end{equation}
where the function $f:\R^{m\times n}\rightarrow\R : \gamma \mapsto f(\gamma)$ is defined as 
\begin{equation}\label{eqn:fgamma}
    f(\gamma)\coloneqq\maxop_{\bM\in\calM}\ \inner{\bV_\gamma,\bM}.
\end{equation}
Here, $\calM=\{\bM:\bM\succeq\bzero {\rm \ and \ }\Omega(\bM) \leq 1\}$ and $\Omega(\cdot)$ is a convex regularizer on the set of positive semi-definite matrices. 
%$\Omega(\cdot)$ may also be an indicator function \commentPJ{(or an indicator function of convex sets)}. 
It should be noted that (\ref{eqn:MahalanobisRobustOT}) is a convex optimization problem. Moreover, by the application of the Sion-Kakutani min-max theorem \cite{sion58}, Problem (\ref{eqn:MahalanobisRobustOT}) can be shown to be equivalent to its dual max-min problem:  $\max_{\bM\in\calM}\min_{\gamma\in\Pi(\bp,\bq)}\inner{\bV_\gamma,\bM}$. 

As discussed in Section~\ref{sec:related}, robust OT distances studied in \cite{paty19a,dhouib20a} can be obtained from (\ref{eqn:MahalanobisRobustOT}) by considering appropriate Schatten-norm based regularizers as $\Omega(\cdot)$. It is well known that Schatten-norm regularizers influence sparsity of the eigenvalues of $\bM$. In contrast, we study novel robust OT formulations based on sparsity promoting regularizers on the entries of $\bM$. A sparse Mahalanobis metric is useful in avoiding spurious feature correlations~\cite{rosales06a,qi09a}. 

%Before presenting the proposed regularizations on $\bM$, we also briefly discuss a common strategy for optimizing (\ref{eqn:MahalanobisRobustOT}) using iterative first-order methods. 

%First-order methods for solving (\ref{eqn:MahalanobisRobustOT}) requires computing the (sub-)gradient $\nabla f(\gamma)|_{\gamma=\gamma^{i}}$, which can be obtained in terms of an optimal solution $\bM^{*}(\gamma^{i})$ of (\ref{eqn:fgamma}) by using the Danskin's theorem \cite{bertsekas1995nonlinear}. Since (\ref{eqn:fgamma}) involves the positive semi-definite constraint, computing $\bM^{*}(\gamma)$ usually involves costly eigendecomposition (or equivalent operations) of $d\times d$ matrices. However, for the proposed family of regularizers $\Omega(\cdot)$, we show that one can drop the symmetric positive definite constraint in (\ref{eqn:fgamma}) as the optimal solution $\bM^{*}(\gamma)$ of the resulting problem automatically satisfies $\bM^{*}(\gamma) \succeq \bzero$. This considerably simplifies our optimization methodology for the proposed formulations. We discuss the proposed regularizers and the  corresponding $\bM^{*}(\gamma)$ in the following sections. 

%and optimized the following max-min problem:
%\begin{equation}\label{eqn:MahalanobisRobustOTmaxmin}
%     {\rm RKP}(\Pi,\calM) =  \maxop_{\bM\in\calM}\minop_{\gamma\in\Pi(\mu_1,\mu_2)}\ \inner{\bV_\gamma,\bM}.
% \end{equation}

%A key benefit of optimizing the max-min formulation (\ref{eqn:MahalanobisRobustOTmaxmin}) is that the inner problem in $\gamma$ can be solved efficiently via the Sinkhorn-Knopp algorithm by adding the negative entropy regularization \cite{cuturi13a}. Thus, the (sub-)gradient \cite{paty19a} or the linear inequalities corresponding to refinement of the feasible set \cite{dhouib20a} may be computed efficiently. However, the outer optimization problem involves enforcing the positive semi-definite constraints, which typically involves costly eigendecomposition operation of $d\times d$ matrix. 


%Let $\bC$ be a given cost matrix imputed with an unknown noise  $\bN\in\R^{m\times n}$. The noise is assumed to from a family characterized by $\Omega(\bN)\leq 1$, where $\Omega: \R^{m\times n}\rightarrow \R_{+}$ is a regularization function. We begin with the setting when an additive noise influences the cost.

% \textbf{Earth-mover distance (EMD)}: The vanilla OT formulation 
% \begin{equation}\label{eqn:emd}
%  \min_{\gamma\in\Pi}  \inner{\gamma,\hat{\bC}}
% \end{equation}
% may be reformulated in the minimax OT setting by choosing $\Omega(\bN)=\max_{(i,j)}\{\bN_{11},\ldots,\bN_{mn}\}$, i.e., 
% \begin{equation}
%  \min_{\gamma\in\Pi}\ \max_{\bN}\ \inner{\gamma,\hat{\bC}+\bN} - \max_{(i,j)}\{\bN_{11},\ldots,\bN_{mn}\}.
% \end{equation}
% The regularization $\Omega(\bN)\leq 1$ implies that the entries of matrix $\bN$ are upper bounded. 

% \textbf{Sinkhorn distance (dual-Sinkhorn divergence)}: \cite{cuturi13a} introduced the entropy regularization in the optimal transport objective to smoothen the objective and have computational benefits. The resulting distance is termed as the Sinkhorn distance (dual-Sinkhorn divergence), which is computed by solving the following OT problem:
% \begin{equation}\label{eqn:sinkhorn}
%  \min_{\gamma\in\Pi}  \inner{\gamma,\hat{\bC}} + \delta\sum_{ij}\gamma_{ij}\ln{\gamma_{ij}}.
% \end{equation}
% The Sinkhorn distance formulation (\ref{eqn:sinkhorn}) can be equivalently reformulated in the minimax framework (\ref{eqn:minimaxGeneralAdditiveNoise}) by setting $\Omega(\bN)=\delta\ln\left(\sum_{ij}e^{\frac{\bN_{ij}}{\delta}}\right)$, i.e., the log-sum-exp function over the entries of the matrix $\bN$. It should be noted that the log-sum-exp function is a smooth approximation of the maximum function. The latter is employed as the regularizer to reformulate the EMD formulation with the minimax OT framework. 

% \textbf{Element-wise $p$-norm regularization}: \cite{blondel18a} considered the squared $2$-norm regularization over the coupling $\gamma$, with the aim of obtaining truly sparse transportation plan (and which may be computed efficiently). The general squared $p$-norm regularized OT formulation ($p\geq1$) may be written as:
% \begin{equation}\label{eqn:squaredPnorm}
%  \min_{\gamma\in\Pi}  \inner{\gamma,\hat{\bC}} + \delta(\sum_{ij}|\gamma_{ij}|^p)^{2/p}.
% \end{equation}
% Problem (\ref{eqn:squaredPnorm}) can be equivalently reformulated in the minimax framework (\ref{eqn:minimaxGeneralAdditiveNoise}) by setting $\Omega(\bN)=\frac{1}{\delta}(\sum_{ij}|\bN_{ij}|^q)^{2/q}$, where $q$ is the dual-norm of $p$, i.e., $\frac{1}{p} + \frac{1}{q} = 1$. 

% \textbf{Schatten $p$-norm regularization}: A nuclear-norm (Schatten $1$-norm) regularization over the coupling $\gamma$ promotes a low-rank representation of the transport plan $\gamma$. Recently,   a low-rank factored transport plan $\gamma$ has been proposed in \cite{forrow19a}. The general Schatten $p$-norm ($p\geq 1$) regularized on OT formulation may be written as
% \begin{equation}\label{eqn:squaredSchattenPnorm}
%  \min_{\gamma\in\Pi}  \inner{\gamma,\hat{\bC}} + \delta\norm{\gamma}_{*p}^2,
% \end{equation}
% where $\norm{\cdot}_{*p}$ denotes the Schatten $p$-norm regularizer for a matrix. Problem (\ref{eqn:squaredSchattenPnorm}) may be equivalently reformulated within the minimax OT framework (\ref{eqn:minimaxGeneralAdditiveNoise}) by choosing $\Omega(\bN)=\frac{1}{\delta}\norm{\bN}_{*q}^2$, where $q$ is the dual-norm of $p$. 

% \subsection{Space of affine transformations}
% The next consider set of affine transformations of the cost matrices:
% $$\CC_{\textup{aff}}=\{\A(\hat{\bC}): \A:\R^{m\times n}\rightarrow\R^{m\times n} \textup{ is a linear operator};\Omega(\A)\leq 1 \},$$
% where $\Omega: \R^{m\times n}\rightarrow \R_{+}$ is a regularization function. The minimax OT problem that learns a robust transport plan over the set of cost functions $\CC_{\textup{aff}}$ may be written as:
% \begin{equation}\label{eqn:minimaxGeneralAffineNoise1}
%  \min_{\gamma\in\Pi}\ \max_{\bC\in\CC_{\textup{aff}}}\  \inner{\gamma,\bC}.
% \end{equation}
% The linear operator $\A$ may be parameterized in a number of ways. For instance, if we consider its form as $\A(\hat{\bC})=\hat{\bC}\bN$ and re-write the above in an equivalent Tikhonov form, we get the following optimization problem:  
% \begin{equation}\label{eqn:minimaxGeneralMultiplicativeNoise}
%  \min_{\gamma\in\Pi} \max_{\bN} \inner{\gamma,\hat{\bC}
% \bN} - \Omega(\bN).
% \end{equation} 
% Using the Fenchel duality theory, the optimization problem in (\ref{eqn:minimaxGeneralMultiplicativeNoise}) may be equivalently reformulated as 
% \begin{equation}\label{eqn:minGeneralMultiplicativeRegularizer}
%  \min_{\gamma\in\Pi}\ \Omega^{*}(\hat{\bC}^\top\gamma).
% \end{equation}
% Similarly, we may parameterize $\A(\hat{\bC})=\bC\odot\bN$, where $\odot$ denote the element-wise product (Hadamard product). Element-wise imputation of the given cost matrix may be useful in modeling scenarios where the importance of the $(i,j)$-th source-target pair is being varied. Then, problem (\ref{eqn:minimaxGeneralAffineNoise1}) may be equivalently reformulated as 
% \begin{equation}\label{eqn:minGeneralHadamardRegularizer}
%  \min_{\gamma\in\Pi}\ \Omega^{*}(\bC\odot\gamma). 
% \end{equation}


%\subsection{Robust $2$-Wasserstein distances}

%Note that one alternative to solve for the minimax OT $RKP(\Pi,\CC)$ with the above class of Mahalanobis cost functions is to get a closed-form expression of $\bM$ in terms of $\gamma$ and thus only solve for $\gamma$. However, this is computationally intensive (except probably for $p=2$) since it involves Schatten $q$-norm terms of $V_\gamma$ (note that $\bM\succeq0)$

%In the previous sections, we analyzed the setting in which noise imputes a generic cost function in the minimax OT framework. We now discuss a novel family of multiplicative noise in the popular $2$-Wasserstein distance setting (\ref{eqn:W22distance}), i.e., when the cost function is the squared Euclidean distance. 

\subsection{Element-wise $p$-norm regularization on $\bM$}\label{sec:p_norm}

We begin by discussing the element-wise $p$-norm regularization on the Mahalanobis metric $\bM$: 
$\calM=\{\bM:\bM\succeq\bzero {\rm \ and \ } \norm{\bM}_{p}\leq1\}$ in (\ref{eqn:fgamma}), where $\norm{\bM}_{p}=(\sum_{ij} |\bM_{ij}|^p)^{\frac{1}{p}}$. For $p$ in between $1$ and $2$, the entry-wise $p$-norm regularization induces a sparse structure on the metric $\bM$. This family of element-wise $p$-norm  regularizers includes the popular Frobenius norm at $p=2$. The following result provides an efficient reformulation of the robust OT problem (\ref{eqn:MahalanobisRobustOT}).

% with the above defined $\calM$ for a subset of the element-wise $p$-norm regularizers on $\bM$. 


% Hence, the proposed regularization on the metric $\bM$ learns appropriate weights to the individual components of $\bV_\gamma$. In contrast, the ${{\rm W}}_2^2$ distance, defined in (\ref{eqn:W22distance}), has $\bM=\bI$, which enforces the first-order displacements to be uncorrelated and have unit variance. This may be a strong assumption in real-word applications.



%The following theorem proposes an equivalent reformulation of the robust OT problem (\ref{eqn:MahalanobisRobustOT}) when the Mahalanobis metric is regularized with element-wise $p$-norm:
\begin{Thm}\label{thm:p-norm}
Consider Problem (\ref{eqn:MahalanobisRobustOT}) with $\calM=\{\bM:\bM\succeq\bzero {\rm \ and \ } \norm{\bM}_p\leq1\}$, $p=\frac{2k}{2k-1}$, and $k\in\mathbb{N}$. Then, (\ref{eqn:MahalanobisRobustOT}) is equivalent to the following optimization problem:
%Let $k\in\mathbb{N}$, $p=\frac{2k}{2k-1}$, and  $\calM=\{\bM:\bM\succeq\bzero {\rm \ and \ } \norm{\bM}_p\leq1\}$. Consider the optimization problem
\begin{equation}\label{eqn:proposed-p-norm-min}
%\begin{array}{lll}
%{\rm RKP}(\Pi,\D) & = & 
{{\rm W}}_{{\rm P}}(\bp,\bq)\coloneqq\minop_{\gamma\in\Pi(\bp,\bq)}\ \norm{\bV_\gamma}_{2k},
%\minop_{\gamma\in\Pi}\ \frac{1}{2k}\left(\frac{2k-1}{2k\lambda}\right)^{2k-1} \sum\limits_{s,t} \bV_\gamma(s,t)^{2k},
%\end{array}
\end{equation}
where $\bV_\gamma=\sum_{ij} (\bs_i-\bt_j)(\bs_i-\bt_j)^\top \gamma_{ij}$. For a given $\gamma\in\Pi(\bp,\bq)$, the optimal solution of (\ref{eqn:fgamma}) is $\bM^{*} (\gamma) =\norm{\bV_{\gamma}}_{2k}^{1-2k}(\bV_{\gamma})^{\circ(2k-1)}$, where $\bA^{\circ (k)}$ denotes the $k$-th Hadamard power of a matrix $\bA$.
% Then, the following statements hold.
% \begin{enumerate}
%     %\item (\ref{eqn:proposed-p-norm-min}) is a convex optimization problem. 
%     \item Problem (\ref{eqn:proposed-p-norm-min}) is a dual of  (\ref{eqn:MahalanobisRobustOT}) and the objectives of (\ref{eqn:MahalanobisRobustOT}) and  (\ref{eqn:proposed-p-norm-min}) are equal at optimality.
%     \item For a given $\gamma\in\Pi(\bp,\bq)$, the optimal solution of (\ref{eqn:fgamma}) is $\bM^{*} (\gamma) =\norm{\bV_{\gamma}}_{2k}^{1-2k}(\bV_{\gamma})^{\circ(2k-1)}$, where $\bA^{\circ (k)}$ denotes the $k$-th Hadamard power of a matrix $\bA$.
%     %, i.e., $\bA^{\circ (k)}(s,t)=\bA(s,t)^k$. 
%     %\item Let $\gamma^{*}$ denote an optimal solution of (\ref{eqn:proposed-p-norm-min}). Then $(\gamma^{*},\bM^{*})$ is an optimal solution of (\ref{eqn:MahalanobisRobustOT}), where $\bM^{*}(s,t)=\left(\frac{2k-1}{2k\lambda}\right)^{2k-1} \bV_{\gamma}(s,t)^{2k-1}$. 
% \end{enumerate}
%Then, the following problem (\ref{eqn:proposed-p-norm-min}) is a dual of ${\rm RKP}(\Pi,\calM)$ in (\ref{eqn:MahalanobisRobustOT}) and the objectives of (\ref{eqn:MahalanobisRobustOT}) and (\ref{eqn:proposed-p-norm-min}) are equal at optimality:
\end{Thm}

% \begin{proof}
% The proof is in Appendix \ref{supp:sec:proof_pnorm}. 
% \end{proof}



%The proposed robust OT formulation is as follows:
% \begin{equation}\label{eqn:proposed-minimax}
% {\rm RKP}(\Pi,\D) =  \minop_{\gamma\in\Pi} \maxop_{\bM\succeq \bzero} \inner{\bV_\gamma,\bM} - \lambda \sum\limits_{ij} |\bM_{ij}|^p.
% \end{equation}

% An optimal solution $\gamma^{*}$ of (\ref{eqn:proposed-p-norm-min}) is also an optimal solution the problem:
% \begin{equation}\label{eqn:proposed-p-norm-min-2}
% {{\rm W}}_{{\rm P}}^{2k}=\minop_{\gamma\in\Pi(\mu_1,\mu_2)}\ \norm{\bV_\gamma}_{2k}^{2k}.
% \end{equation}
% From an optimization perspective the gradient expression for (\ref{eqn:proposed-p-norm-min-2}) is simpler than that of  (\ref{eqn:proposed-p-norm-min}). 

From Theorem~\ref{thm:p-norm}, it follows that for a given $\gamma$, the optimal $\bM^{*}(\gamma)$ is an element-wise function of the matrix $\bV_\gamma$. An implication is that the computation of $\bM^*(\gamma)$ costs $O(d^2)$. 

%\textbf{Computing optimization ingredients efficiently}: 

% \subsection{The material below goes to supplementary}
% We begin by noting that that $\bV_\gamma = \bZ {\rm Diag}({\rm vec}(\gamma)) \bZ^\top$, where $\bZ$ is a $d\times mn$ matrix with $(i,j)$-th column as $(\bx_i-\by_j)$, ${\rm Diag}(\cdot)$ acts on a vector and outputs the corresponding diagonal matrix, and ${\rm vec}(\cdot)$ vectorizes a matrix in the column-major order. The Euclidean gradient of (\ref{eqn:proposed-p-norm-min-2}) is ${\rm vec}^{-1}({\rm diag}(\bZ^\top\bV_\gamma^{\circ(2k-1)}\bZ))$, where ${\rm diag}(\cdot)$ extracts the diagonal (vector) of a square matrix. \commentPJ{The Euclidean Hessian along a search direction $\dot{\gamma}$ is $({2k-1}){\rm vec}^{-1}({\rm diag}(\bZ^\top(\bV_\gamma^{\circ (2k-2)} \odot(\bZ {\rm Diag}({\rm vec}(\dot{\gamma})) \bZ^\top))\bZ))$.}

%{\color{red}\textbf{\#1 Some bounds for the above norm:} Lets consider the original cost $c(\bx,\by)=(\bx-\by)^\top\bI(\bx-\by)$ and its robust variant:  $c_\bM(\bx,\by)=(\bx-\by)^\top(d\bM)(\bx-\by)$. This implies that instead of $\bx$ we are considering data points of the form $\sqrt{d}\bM^\frac{1}{2}\bx$. From Holders inequality, we get $\bx^\top\bM\bx=\inner{\bM,\bx\bx^\top}\leq\norm{\bM}_p\norm{\bx\bx^\top}_q$, where the norms in the RHS is element-wise norms. Now $\norm{\bx\bx^\top}_2=\norm{\bx\bx^\top}_F=\sqrt{\trace(\bx\bx^\top\bx\bx^\top)}=\norm{\bx}^2$.}

%This class of cost functions has a different property than the class discussed in \cite{dhouib20a,paty19a}. The proposed family of robust Wasserstein distances performs feature selection (to be expanded further). 
%The optimization problem corresponding to ${\rm RKP}(\Pi,\D)$ may be written, in Tikhonov form, as:
%We have the following result on the proposed ${\rm RKP}(\Pi,\D)$: 

%It should be noted that the above problem is convex with respect to $\gamma$ (maxima over convex functions is convex). 
%In the following theorem, we propose an equivalent reformulation of the proposed minimax OT problem. 




% The problem (\ref{eqn:proposed-p-norm-min-2}) can be reformulated as
% \begin{equation}\label{eqn:proposed-min-compact}
% \begin{array}{lll}
% {\rm RKP}(\Pi,\D) & = & \minop_{\gamma\in\Pi}  \bone^\top\bv_\gamma^{2k},
% \end{array}
% \end{equation}
% where $\bv_\gamma$ is the vectorization of $\bV_\gamma$, i.e., $\bv_\gamma = {\rm vec}(\bV_\gamma)$. Also, $\bv_\gamma$ can be compactly written as $\bv_\gamma = \bP {\rm vec}(\gamma)$, where $\bP = [{\rm vec}((\bx_i-\by_j)(\bx_i-\by_j)^\top)]$ is a matrix of size $d^2 \times mn$ and $\rm{vec}$ is the vectorization operation. The Euclidean gradient is $2k{\rm vec}^{-1} ( \bP^\top \bv_\gamma^{2k-1} )$, where ${\rm vec}^{-1}$ is the reshaping of the vector back to the matrix dimensions. 
%The Euclidean Hessian along a search direction $\dot{\gamma}$ is $({2k-1})\left(\frac{2k-1}{2k\lambda}\right)^{2k-1} {\rm vec}^{-1}(\bP^\top ((\bv_\gamma^{2k-2})\odot(\bP {\rm vec}(\dot{\gamma}) )))$. 

% Another way to reformulate (\ref{eqn:proposed-min}) is by observing $\bV_\gamma = \bZ {\rm Diag}({\rm vec}(\gamma)) \bZ^\top$, where $\bZ$ is a $d\times mn$ matrix by stacking $(\bx_i - \by_j)$ side by side for all pairs and ${\rm Diag}$ acts on a vector and outputs a diagonal matrix. The Euclidean gradient is $\left(\frac{2k-1}{2k\lambda}\right)^{2k-1}  {\rm vec}^{-1}({\rm diag}(\bZ^\top\bV_\gamma^{2k-1}\bZ))$, where ${\rm diag}()$ extracts the diagonal of a square matrix. The Euclidean Hessian along a search direction $\dot{\gamma}$ is $({2k-1})\left(\frac{2k-1}{2k\lambda}\right)^{2k-1} {\rm vec}^{-1}({\rm diag}(\bZ^\top(\bV_\gamma^{2k-2} \odot(\bZ {\rm Diag}({\rm vec}(\dot{\gamma})) \bZ^\top))\bZ))$.


%\textbf{Special case of Frobenius norm regularization on $\bM$}: For $k=1$, we have the following simplified convex quadratic objective for the computing ${\rm W}_{{\rm E}}^{2k}$ in problem (\ref{eqn:proposed-p-norm-min-2}): $\norm{\bV_\gamma}_2^2={\rm vec}(\gamma)^\top \bA {\rm vec}(\gamma)$, where $\bA=(\bZ^\top\bZ)\odot (\bZ^\top\bZ)$ and $\odot$ denotes the Hadamard product. 
%\textbf{Special case of Frobenius norm regularization on $\bM$}: For $k=1$, we have the following simplified convex quadratic objective for the computing ${\rm W}_{{\rm E}}^{2k}$: $\norm{\bV_\gamma}_2^2={\rm vec}(\gamma)^\top \bA {\rm vec}(\gamma)$, where $\bA=(\bZ^\top\bZ)\odot (\bZ^\top\bZ)$ and $\odot$ denotes the Hadamard product. 
%In this special case of $p=2$, the proposed formulation is equivalent to the Schatten $2$-norm formulation discussed in \cite{dhouib20a}. However, \cite{dhouib20a} only discusses the general algorithm and does not explore such simplifications. 




\subsection{KL-divergence regularization on $\bM$}\label{sec:KL}


We next consider the generalized KL-divergence regularization on the metric $\bM$, i.e., $\calM=\{\bM:\bM\succeq\bzero;{{\rm D}_{\rm KL}}(\bM,\bM_0)\leq 1\}$, where ${{\rm D}_{\rm KL}}(\bM,\bM_0)=\sum_{a,b} \bM_{ab}(\ln{\left(\bM_{ab}/{\bM_0}_{ab}\right)})-(\bM_{ab} - {\bM_{0}}_{ab})$ denotes the Bregman distance, with negative entropy as the distance-generating function, between the matrices $\bM$ and $\bM_0\succeq\bzero$. Here, $\bM_0$ is a given symmetric PSD matrix, which may be useful in introducing prior domain knowledge (e.g., a block diagonal matrix $\bM_0$ ensures grouping of features). 
%and $\ln(\cdot)$ is the natural logarithm operation. 
%A default choice of $\bM_0$ is  $\bM_0=\bone\bone^\top$, where all the features are equally correlated (similar) with each other. 
The function $f(\gamma)$ in (\ref{eqn:fgamma}) with the above defined $\calM$ may be expressed equivalently in the Tikhonov form as
%This regularization ensures that the entries of $\bM$ are positive. Hence, the domain of $\bM$ is the set of positive-definite matrices with positive entries. 
\begin{equation}\label{eqn:proposed-minimax-kl-divergence}
f(\gamma) = \maxop_{\bM\succeq \bzero}\  \inner{\bV_\gamma,\bM}-\lambda_{\bM} {{\rm D}_{\rm KL}}(\bM,\bM_0),
\end{equation}
% \begin{equation}\label{eqn:proposed-minimax-kl-divergence}
% {{\rm W}}_{{\rm KL}}(\mu_1,\mu_2) = \minop_{\gamma\in\Pi} \maxop_{\bM\succeq \bzero}\  \inner{\bV_\gamma,\bM}- \lambda_{\bM} {{\rm D}_{\rm KL}}(\bM,\bM_0),
% \end{equation}
where $\lambda_{\bM}>0$ is a regularization parameter. The following result provides an efficient reformulation of the KL-divergence regularized robust OT problem. 
\begin{Thm}\label{thm:kl-regularization}
%Consider the KL-divergence regularized robust OT problem (\ref{eqn:MahalanobisRobustOT}), where $f(\gamma)$ is as defined in (\ref{eqn:proposed-minimax-kl-divergence}). 
The following problem is an equivalent dual of the convex problem (\ref{eqn:MahalanobisRobustOT}) where $f(\gamma)$ is as defined in (\ref{eqn:proposed-minimax-kl-divergence}):
\begin{equation}\label{eqn:proposed-min-kl-divergence}
\begin{array}{lll}
%W_{KL}(\mu_1,\mu_2) = \minop_{\gamma\in\Pi} \lambda \sum\limits_{s,t} \bM_0(s,t)(e^{\bV_\gamma(s,t)/\lambda}-1).
{{\rm W}}_{{\rm KL}}(\bp,\bq) \\
= \minop_{\gamma\in\Pi(\bp,\bq)} \lambda_{\bM} \bone^\top( \bM_0\odot e^{\circ (\bV_\gamma/\lambda_{\bM})} - \bM_0)\bone,
\end{array}
\end{equation}
where $e^{\circ\bA}$ denotes the Hadamard exponential (element-wise exponential) of a matrix $\bA$ and $\odot$ denotes the Hadamard product (element-wise product). For a given $\gamma\in\Pi(\bp,\bq)$, the optimal solution of  (\ref{eqn:proposed-minimax-kl-divergence}) is  $\bM^{*}(\gamma)=\bM_0\odot e^{\circ (\bV_{\gamma}/\lambda_{\bM})}$. 
\end{Thm}
% \begin{proof}
% We first characterize the relaxed unconstrained (i.e., without the PSD constraint) solution of (\ref{eqn:proposed-minimax-kl-divergence}), which is $\bM^{*}(\gamma)=\bM_0\odot e^{\circ (\bV_{\gamma}/\lambda_{\bM})}$. As element-wise exponential operation on symmetric PSD matrices preserves positive semi-definiteness, i.e., $\bM^{*}(\gamma)=\bM_0\odot e^{\circ (\bV_{\gamma}/\lambda_{\bM})}$ is also PSD, implying that this is also the optimal solution of (\ref{eqn:proposed-minimax-kl-divergence}). Putting $\bM^{*}(\gamma)$ in the objective function of (\ref{eqn:proposed-minimax-kl-divergence}) leads to (\ref{eqn:proposed-min-kl-divergence}).
% \end{proof}



The proposed KL-regularization based OT formulation (\ref{eqn:proposed-minimax-kl-divergence}) is closely related to selecting discriminative features that maximize the optimal transport distance between two distributions. We formalize this in our next result. 
\begin{Lem}\label{lemma:feature-selection}
Let $\gamma^{*}$ be the solution of (\ref{eqn:proposed-min-kl-divergence}) with $\bM_0=\bI$. Then, $\gamma^{*}$ is also the solution of the following robust OT formulation:
\begin{equation}\label{eqn:feature-selection}
%\maxop_{\bm\in\Delta_d}\ \minop_{\gamma\in\Pi(\mu_1,\mu_2)}  \inner{\bV_\gamma,\bM}-\lambda_{\bM} {{\rm D}_{\rm KL}}(\bM,\bI),
\minop_{\gamma\in\Pi(\bp,\bq)}\ \maxop_{\bm\in\Delta_d} \inner{\gamma,\bC_{\bm}}-\lambda_{\bm} {{\rm D}_{\rm KL}}(\bm,\bone),
\end{equation}
%$\bM$ is the diagonal matrix corresponding to the vector $\bm$,  $\Delta_d$ is the $d$-dimensional simplex and 
where $\bC_{\bm}$ is the ground cost matrix corresponding to the function $c_{\bm}(\bs_i,\bt_j)=\sum_{a=1}^d \bm_a (\bs_{ia}-\bt_{ja})^2$. Here, $\bs_{ia}$ and $\bt_{ja}$ denote the $a$-th coordinate of $\bs_i$ and $\bt_j$, respectively. 
\end{Lem}
%The ground cost function corresponding to (\ref{eqn:feature-selection}), as a function of $\bm$ (or equivalently $\bM$), is $c_{\bM}(\bs_i,\bt_j)=\sum_{l=1}^d \bm_l (\bs_{il}-\bt_{jl})^2$, where $\bs_{il}$ and $\bt_{jl}$ denote the $l$-th coordinate of the data points $\bs_i$ and $\bt_j$, respectively. 

% \begin{proof}
% The proof is in Appendix \ref{supp:sec:proof_simplex}.
% \end{proof}

The simplex constraint over feature weights in (\ref{eqn:feature-selection}) results in feature selection. %selecting features that maximize the OT distance 
%It can be observed that if the learned weight of the $l$-th feature is zero, i.e., $\bm_l=0$, the $l$-th feature does not influence the computation of  (\ref{eqn:feature-selection}). 
Thus, the proposed robust OT formulation (\ref{eqn:proposed-min-kl-divergence}) may equivalently be viewed as a robust OT formulation involving feature selection when $\bM_0=\bI$. 
%From Lemma~\ref{lemma:feature-selection}, the transport plan $\gamma^{*}$ learned in (\ref{eqn:proposed-min-kl-divergence}) is also an optimal solution of (\ref{eqn:feature-selection}), which may be viewed as a minimax OT problem involving feature selection. 
%Feature selection in the OT setting has also been explored in a concurrent work by Petrovich et al. \cite{petrovich20a}.


%Since $\bM$ is restricted to a non-negative diagonal matrix in (\ref{eqn:feature-selection}), it simply reweigh the $i-$th input features of source and target samples by the scalar $\bm_i$

% It should be noted that the optimal solution $\gamma^{*}$ of (\ref{eqn:proposed-min-kl-divergence}) with $\bM_0=\bone\bone^\top$ is also the optimal solution of the problem:
% \begin{equation}\label{eqn:proposed-min-log-sum-exp}
% %\begin{array}{lll}
% {{\rm W}}_{{\rm S}}(\mu_1,\mu_2)=\minop_{\gamma\in\Pi(\mu_1,\mu_2)} \lambda \log{\left(\sum\limits_{s,t} e^{\bV_\gamma(s,t)/\lambda}\right)}.
% %\end{array}
% \end{equation}
% The objective in (\ref{eqn:proposed-min-log-sum-exp}) is a log-sum-exp function on the entries of the matrix $\bV_\gamma$, which is a smooth approximation of the maximum function. Thus, the optimal $\gamma^{*}$ in (\ref{eqn:proposed-min-log-sum-exp}) minimizes (a smooth approximation of) the maximum over the  entries of $\bV_\gamma$. Interestingly, problem (\ref{eqn:proposed-min-log-sum-exp}) is equivalent to the robust OT problem (\ref{eqn:MahalanobisRobustOT}) with $f(\gamma)$ defined as 
% \begin{equation}\label{eqn:proposed-minimax-log-sum-exp}
% f(\gamma) =  \maxop_{\bM\in\calM} \inner{\bV_\gamma,\bM} - \lambda {{\rm D}_{\rm KL}}(\bM,\bone\bone^\top),
% \end{equation}
% where $\calM=\{\bM:\bM\succeq \bzero;\bM>\bzero;\bone^\top\bM\bone=1\}$. We observe that problem (\ref{eqn:proposed-minimax-log-sum-exp}) learns a positive semi-definite Mahalanobis metric whose entries lies on a $(mn-1)$-dimensional simplex \commentPJ{(without a boundary)}. 
%We next analyze the doubly-stochastic structure on $\bM$. 


\subsection{Doubly-stochastic regularization on $\bM$}\label{sec:doubly_stochastic}

We further study the KL-regularization based robust OT objective (\ref{eqn:proposed-minimax-kl-divergence}) with a doubly-stochastic constraint on the Mahalanobis metric $\bM$, i.e.,
\begin{equation}\label{eqn:proposed-doubly-stochastic}
    {\rm W}_{\rm DS}(\bp,\bq) = \minop_{\gamma\in\Pi(\bp,\bq)} f(\gamma),
\end{equation}
where
\begin{equation}\label{eqn:proposed-minimax-doubly-stochastic}
%{{\rm W}}_{{\rm DS}}(\mu_1,\mu_2) = \minop_{\gamma\in\Pi} \maxop_{\bM\in\calM}\ \inner{\bV_\gamma,\bM},
f(\gamma) = \maxop_{\bM\in\calM}\ \inner{\bV_\gamma,\bM} - \lambda_{\bM}{{\rm D}_{\rm KL}}(\bM,\bM_0)
\end{equation}
and $\calM=\{\bM:\bM\succeq\bzero ,\bM \geq\bzero,\bM\bone=\bone,\bM^\top\bone=\bone\}$. 
Learning a doubly-stochastic Mahalanobis metric is of interest in  applications such as graph clustering and community detection \cite{zass06a,wang16a,douik18a}. %arora11a,douik2019manifold
Since $\bM$ is a symmetric PSD matrix, $\bM\bone=\bone \Leftrightarrow \bM^\top\bone=\bone$. 
%In our case, the doubly-stochastic constraint on $\bM$ allows to capture natural associations among various components of the second-order moment matrix $\bV_\gamma$. 


In general, optimization over the set of symmetric PSD doubly-stochastic matrices is non trivial and computationally challenging. By exploiting the problem structure, however, we show that (\ref{eqn:proposed-minimax-doubly-stochastic}) can be solved efficiently. %by adding a small KL-divergence regularization. To this end, we propose to solve for
%\begin{equation}\label{eqn:proposed-max-doubly-stochastic-regularized}
%\Tilde{f}(\gamma) =
%\maxop_{\bM\in\calM}\ \inner{\bV_\gamma,\bM} - \lambda_{\bM}{{\rm D}_{\rm %KL}}(\bM,\bM_0),
%\end{equation}
%where $\lambda_{\bM}>0$ is a small regularization parameter and $\bM_0$ is a symmetric positive semi-definite prior which is also element-wise positive. 
% Our next result characterizes {the optimal} solution of (\ref{eqn:proposed-minimax-doubly-stochastic}). 
\begin{Thm}\label{thm:doubly-stochastic-regularization}
For a given $\gamma\in\Pi(\bp,\bq)$, {the optimal} solution of (\ref{eqn:proposed-minimax-doubly-stochastic}) has the form $\bM^{*}(\gamma)=\bD\left( \bM_0 \odot e^{\circ(\bV_\gamma/\lambda_{\bM})}\right)\bD$, where $\bD$ is a diagonal matrix with positive entries. The matrix $\bD$ can be computed using the Sinkhorn algorithm \cite{cuturi13a}. 
\end{Thm}

% \begin{proof}
% The proof is in Appendix \ref{supp:sec:proof_DS}.
% \end{proof}





\section{Optimization}\label{sec:optimization}
In this section, we discuss how to solve (\ref{eqn:MahalanobisRobustOT}). But first, we discuss a novel low-dimensional modeling approach that helps reduce the computational burden and is amenable to our proposed regularizations in Section \ref{sec:formulations}.




\subsection{Low-dimensional modeling of $\bM$ with feature grouping} \label{sec:low_dimensional_metric_decomposition}


Section \ref{sec:formulations} discusses several regularizations on the Mahalanobis metric $\bM$ that lead to efficient computation of $\bM^{*}(\gamma)$, i.e., the solution to  (\ref{eqn:fgamma}), requiring $O(d^2)$ computations. This, though linear in the size of $\bM$, may be prohibitive for  high-dimensional data. Here, we discuss a particular low-dimensional modeling technique that addresses this computational issue. We consider our Mahalanobis metric $\bM$ to be of the {\it general} form 
%We propose to \changeBM{decompose} the Mahalanobis metric $\bM$ as follows:
\begin{equation}\label{eqn:factorizeMahalanobis}
    \bM=\bB\otimes\bI_{d_1},
\end{equation}
where $\otimes$ denotes the Kronecker product, $\bI_{d_1}$ is the identity matrix of size $d_1 \times d_1$, and  $\bB\succeq\bzero$ is a $r\times r$ symmetric positive semi-definite matrix with $d=d_1r$, where $r \ll d$. 
The modeling (\ref{eqn:factorizeMahalanobis}) reformulates the objective in (\ref{eqn:fgamma}) as
\begin{equation}\label{eqn:reshaping}
\begin{array}{l}
    \inner{\bV_\gamma,\bB\otimes\bI_{d_1}} = \inner{\sum_{ij}\gamma_{ij}(\bs_i-\bt_j)(\bs_i-\bt_j)^\top,\bB\otimes\bI_{d_1}}\\
    \qquad\qquad\qquad= \inner{\sum_{ij}\gamma_{ij}(\bS_i-\bT_j)^\top(\bS_i-\bT_j),\bB}\\
    \qquad\qquad\qquad= \inner{\bU_\gamma, \bB},
\end{array}
\end{equation}
where $\bS_i$ and $\bT_j$ are $d_1\times r$ matrices obtained by reshaping the vectors $\bs_i$ and $\bt_j$, respectively, and $\bU_\gamma\coloneqq \sum_{ij}\gamma_{ij}(\bS_i-\bT_j)^\top(\bS_i-\bT_j)$. 


We observe that the proposed modeling (\ref{eqn:factorizeMahalanobis}) divides $d$ features into $r$ groups, each with $d_1$ features. Based on (\ref{eqn:reshaping}), the symmetric positive semi-definite matrix $\bB$ may be viewed as a Mahalanobis metric over the {\it feature groups}. In addition, it can be shown that any proposed regularization on the metric $\bM$ (in Section~\ref{sec:formulations}) transforms into an equivalent regularization on the ``group'' metric $\bB$. Equivalently, our robust OT problem is with $\gamma$ and 
$\bB$ (and not $\bM$). In case there is no feature grouping ($d_1 = 1$), learning of $\bB$ is same as $\bM$ and there is no computational benefit.

The function $f(\gamma)$, in the robust optimal transport problem (\ref{eqn:MahalanobisRobustOT}), is equivalently re-written as
\begin{equation}\label{eqn:factorizeMahalanobisRobustOT}
    f(\gamma) = \max_{\bB\in\calB}\ \inner{\bU_\gamma,\bB},
\end{equation}
where $\calB=\{\bB:\bB\succeq\bzero {\rm \ and \ } \Omega(\bB) \leq 1\}$. For the regularizers discussed in Section \ref{sec:formulations}, the computation of the solution $\bB^*(\gamma)$ of (\ref{eqn:factorizeMahalanobisRobustOT}) costs $O(r^2)$. 









\subsection{Frank-Wolfe algorithm for (\ref{eqn:MahalanobisRobustOT})}\label{sec:algorithms}

% The formulations proposed in Section \ref{sec:formulations} are expressed as minimization of a non-linear convex function $f: \Pi \rightarrow \mathbb{R} : \gamma \mapsto f(\gamma)$ over $\Pi(\mu_1, \mu_2)$. Here, the objective function $f$ encapsulates the Mahalanobis metric $\bM$ and is more generically written as $f(\gamma) \coloneqq  \max_{\bM \in \mathcal{M}} \langle \bV_{\gamma},  \bM\rangle$. 


A popular way to solve a convex constrained optimization problem (\ref{eqn:MahalanobisRobustOT}) is with the Frank-Wolfe (FW) algorithm~\cite{jaggi2013revisiting} (also known as the conditional gradient algorithm). It requires solving a constrained linear minimization sub-problem (LMO) at every iteration. The LMO step boils down to solving the standard optimal transport problem (\ref{eqn:optimal-transport-discrete}). When regularized with an entropy regularization term, the LMO step admits a computationally efficient solution using the popular Sinkhorn algorithm \cite{cuturi13a}. The FW algorithm  for (\ref{eqn:MahalanobisRobustOT}) is shown in Algorithm \ref{alg:FW}, which only involves the gradient of the function.



\begin{algorithm}[tb]
   \caption{Proposed FW algorithm for (\ref{eqn:MahalanobisRobustOT})}
   \label{alg:FW}
   {%\footnotesize
    %\begin{tabular}{ l | l }
  {\bfseries Input:} Source distribution's samples $\{\bs_i\}_{i=1}^m\in\R^{d}$ and target distribution's samples $\{\bt_j\}_{j=1}^n\in\R^{d}$. 
  
  {\bfseries Initialize:} $\gamma_0 \in \Pi(\mu_1, \mu_2)$. 
   
  {\bfseries for} $t = 0\ldots T$ {\bfseries do} 
  
  \qquad Compute $\nabla f_{\gamma}(\gamma_t)$ using Lemma \ref{lemma:gradient_and_directional_derivative}.
  
  
  \qquad LMO step: Compute $\hat{\gamma}_t\coloneqq \argmin_{\beta \in \Pi(\bp,\bq)} \langle \beta, \nabla f_{\gamma}(\gamma_t)\rangle$.
  
  
  \qquad Update $\gamma_{t+1} = (1-\theta)\gamma_t + \theta \hat{\gamma}_t$ for $\theta = \frac{2}{t+2}$.
 
  {\bfseries end for}

{\bfseries Output:} $\gamma^*$ and $\bM^* = \bM^*(\gamma^*)$.
%    \end{tabular}
    }
\end{algorithm}


We now show the computation of gradient $\nabla_{\gamma} f$ of (\ref{eqn:MahalanobisRobustOT}). We begin by noting that $\bV_\gamma = \bZ {\rm Diag}({\rm vec}(\gamma)) \bZ^\top$, where $\bZ$ is a $d\times mn$ matrix with $(i,j)$-th column as $(\bs_i-\bt_j)$, ${\rm Diag}(\cdot)$ acts on a vector and outputs the corresponding diagonal matrix, and ${\rm vec}(\cdot)$ vectorizes a matrix in the column-major order. 

\begin{Lem}\label{lemma:gradient_and_directional_derivative}
Let $\bM^*(\gamma_t)$ be the solution of the problem $\maxop_{\bM \in \mathcal{M}} \langle \bV_{\gamma_t},  \bM\rangle$ for a given $\gamma_t \in \Pi(\bp,\bq)$. Then, the gradient $\nabla_{\gamma} f (\gamma_t)$ of $f(\gamma)$ in (\ref{eqn:MahalanobisRobustOT}) with respect to $\gamma$ at $\gamma_t$ is
\begin{equation*}
    \nabla_{\gamma} f(\gamma_t) = {\rm vec}^{-1}({\rm diag}(\bZ^\top \bM^*(\gamma_t)\bZ)), 
\end{equation*}
where ${\rm diag}(\cdot)$ extracts the diagonal (vector) of a square matrix and ${\rm vec}^{-1}$ reshapes a vector into a matrix. 

\end{Lem}
% \begin{proof}
% The proof follows directly from the Danskin's theorem \cite{bertsekas1995nonlinear} and exploits the structure of $\bV_{\gamma}$.
% \end{proof}

For the formulations presented in Section \ref{sec:formulations}, the computation of $\nabla_{\gamma} f$ costs $O(mnd^2)$. 
For the cost function (\ref{eqn:factorizeMahalanobisRobustOT}) obtained with the $r$-dimensional modeling of $\bM$, Lemma \ref{lemma:gradient_and_directional_derivative} can be appropriately modified. In this case, the cost of computation of $\nabla_{\gamma} f $ is $O(mnr^2)$.







% \subsection{Manifold approach}\label{sec:manifold}


% Another approach is by exploiting the fact that $\Pi(\mu_1,\mu_2)$ has a smooth manifold structure for $\gamma > 0$, i.e., strict positivity of the entries of $\gamma$ \cite{douik2019manifold,shi19a}. In particular, we use the Riemannian optimization framework that 
% conceptually translates a constrained optimization problem of the form (\ref{eqn:MahalanobisRobustOT}) into an {\it unconstrained} optimization problem over the manifold $\Pi(\mu_1,\mu_2)$. It allows to build first- and second-order algorithms over $\Pi(\mu_1,\mu_2)$ systematically, thereby allowing to use conjugate gradients and trust-regions algorithms \cite{absil2009optimization,boumal2020intromanifolds}.


% $\Pi(\mu_1,\mu_2)$ is endowed with the {\it Fisher} information metric, as the Riemannian metric, defined as \cite{douik2019manifold,shi19a,sun2015heterogeneous}
% \begin{equation}\label{eqn:Riemannian_metric}
%     \begin{array}{ll}
%          g_{\gamma}(\eta_{\gamma}, \xi_{\gamma}) \coloneqq 
%          \trace((\eta_{\gamma} \odot \xi_{\gamma}) \oslash \gamma),
%     \end{array}
% \end{equation}
% where $\eta_{\gamma}$ are $ \xi_{\gamma}$ tangent vectors belonging to the tangent space $T_{\gamma} \Pi(\mu_1,\mu_2) \coloneqq \{ \zeta_{\gamma} \in \mathbb{R}^{m\times n} : \zeta_{\gamma} \bone = 1/m, \zeta_{\gamma}^\top \bone =  1/n \}$ at $\gamma$. Here, $\odot$ and $\oslash$ are element-wise matrix multiplication and division, respectively. The Riemannian metric (\ref{eqn:Riemannian_metric}) scales the boundary of $\Pi(\mu_1,\mu_2)$ to ``infinity'', i.e., as $\gamma_{ij}$ tends to zero, the inner product tends to infinity, thereby endowing $\Pi(\mu_1,\mu_2)$ with a smooth {\it differentiable} structure. \changeBM{This is in contrast to the FW approach in Section \ref{sec:FW} where an entropy term has to be added explicitly in the LMO step.}


% %It is interesting to note that the Fisher metric (\ref{eqn:Riemannian_metric}) is same as the popular Bures-Wasserstein metric (defined for the manifold of symmetric positive definite matrices) when restricted to positive scalars \cite{bhatia2019bures,malago2018wasserstein}.  


% The Riemannian conjugate (CG) gradient and trust-regions (TR) algorithms require the notions of Riemannian {\it gradient} (the steepest descent direction on the manifold) and {\it Hessian} (the covariant derivative of the Riemannian gradient), which admit simple formulas in terms of $\nabla f$ and its directional derivative ${\rm D} \nabla f(\gamma)[\dot{\gamma}]$, respectively \cite{douik2019manifold,sun2015heterogeneous}. Moving along the manifold is captured with the notion of a {\it retraction} operator (ensures that we always stay on the manifold) which has a well-defined expression using the Sinkhorn-Knopp algorithm \cite{douik2019manifold}.



% %Conceptually, the Riemannian optimization framework translates a constrained optimization problem of the form (\ref{eqn:manifold_optimization}) into {\it unconstrained} optimization over the manifold $\Pi$. Accordingly, standard notions of optimization like gradient (the descent direction of a function on the manifold), Hessian (the second-order derivatives of a function), updates on the manifold (moving along the shortest path on the manifold), and transport of (tangent) vectors are generalized to the manifold space. Those expressions have easy-to-implement numerical formulas for the manifold $\Pi$ given any smooth function $f$ \cite{douik2019manifold}.






 



% \section{Related work}
% For a given $\gamma$, the worst case Mahalanobis metric parameterized cost function with the Schatten $p$-norm regularization is given by \citep[Proposition 1]{dhouib20a}:
% \begin{equation}\label{eqn:schatten-norm}
%     \bM^{*}(\gamma) = \argmax\limits_{\bM\succeq\bzero, \norm{\bM}_{*p}\leq1} \inner{\bV_\gamma,\bM}=\left(\frac{\bV_\gamma}{\norm{\bV_\gamma}_{*q}}\right)^{\frac{q}{p}},
% \end{equation}
% where $\norm{\cdot}_{*p}$ denotes the Schatten $p$-norm and $q$-norm is the dual of $p$-norm. Computing $\bM^{*}(\gamma)$ in (\ref{eqn:schatten-norm}) is relatively simple for $p=\{1,2,\infty\}$ but requires eigenvalue decomposition of the matrix $\bV_\gamma$ for other values of $p$. This is due to the positive semi-definite (PSD) constraint over the matrix $\bM$. In this regard, \cite{dhouib20a} has remarked that \textit{``PSD constraints increase considerably the computational burden of any optimization problem, yet they are necessary for the obtained cost function to be a true metric.''}

% \cite{dhouib20a} also analyze the minimax OT problem where the worst case cost function belongs to a convex hull of a finite number of cost functions. Hence, if $\{c_1,\ldots,c_K\}$ is a given set of cost functions, then the search space of the cost functions is $c=\sum_{i=1}^K \alpha_i c_i$, where $\alpha$ lies on a $K-1$ dimensional simplex polytope ($\sum_i \alpha_i=1, \alpha_i\geq 0\ \forall i$).  


\section{Learning with robust optimal transport loss}\label{sec:ROTloss}

% Optimal transport based distances provide a natural metric on the output space, and hence, can be used as a loss function in learning problems \cite{frogner15a,arjovsky17a}. 
%Specifically, Frogner et al.~\cite{frogner15a} discuss the multi-label classification problem set up where they employ the Wasserstein distance as the loss function. 
We next discuss the suitability of our robust OT distances as a loss function in the discriminative learning setup.  
%We begin by explaining the learning problem setup with ${\rm W}_{\rm ROT}$ as a loss function. 
%We then discuss the qualitative nature of the proposed robust OT distance-based loss functions and present an efficient way to compute the gradient of the robust OT distance loss. 
% Later in Section~\ref{sec:experiments}, we empirically demonstrate the effectiveness of using ${\rm W}_{\rm ROT}$ as loss function in supervised multi-label/multi-class classification problems. 

\subsection{Problem setup}
Consider a multi-label (or multi-class) problem over $L$ labels (classes) and given training instances $\{\bx_j,\by_j\}_{j=1}^N$. Here, $\bx_j\in\R^M$ and $\by_j\in\{0,1\}^L$. The prediction function of $p$-th label is given by the {\it softmax} function
\begin{equation}\label{eqn:softmax}
    h_p(\bx;\bW)=\frac{e^{\inner{\bw_p,\bx}}}{\sum_{l=1}^L e^{\inner{\bw_l,\bx}}},
\end{equation}
where $\bW=[\bw_1,\ldots,\bw_L]$ is the model parameter of the multi-label problem. The prediction function $h(\bx;\bW)$ can be learned via the empirical risk minimization framework. 

Frogner et al.~\cite{frogner15a} propose employing the OT distance (\ref{eqn:optimal-transport-discrete}) as the loss function for multi-label classification problem as follows. For an input $\bx_j$, the prediction function $h(\bx_j;\bW)$ in (\ref{eqn:softmax}) may be viewed as a discrete probability distribution. Similarly, a $0-1$ binary ground-truth label vector $\by_j$ may be transformed into a discrete probability distribution by appropriate normalization: $\hat{\by}_j=\by_j/\by_j^\top \bone$. Given a suitable ground cost metric between the labels, the Wasserstein distance is employed to measure the distance between the prediction $h(\bx_j;\bW)$ and the ground-truth $\hat{\by}_j$. If the labels correspond to real-word entities, then a possible ground cost metric may be obtained from the word embedding vectors corresponding to the labels \cite{bojanowski16a}%mikolov13a
. 

\begin{figure}[t]
\center
\includegraphics[width=.45\textwidth]{draft/figs/RboTvsM22_Siamese+cat_Elephant_kl_1e-2_notype3.pdf}
\caption{Contour plots of various OT distance based loss functions. The labels are \{`Siamese$\_$cat', `Elephant', `Persian$\_$cat'\}, with `Persian$\_$cat' as the true label. The plots show the relative loss incurred by various possible predictions of the form $\bh=[x,y,1-x-y]^\top$, where $0\leq x,y\leq1$ and $x+y\leq 1$. We observe linear contours for the ${\rm W}_2^2$ loss function while non-linear contours for the proposed robust OT loss functions: ${\rm W}_{\rm P}$ with $k=1$, ${\rm W}_{\rm KL}$, and ${\rm W}_{\rm DS}$. The robust OT loss functions relatively penalize `Siamese$\_$cat' lesser than `Elephant', i.e., more lighter color in the feasible $x>y$ regions in plots (b), (c), and (d) than in plot (a). }\label{fig:cce}
\end{figure}


% \begin{figure}[t]
% \center
% \includegraphics[width=.5\textwidth]{figs/RboTvsM22_Blue+whale_Elephant_kl_1e-2.pdf}
% \caption{Contour plots of various OT distance based loss functions. The labels are \{`Blue$\_$whale', `Elephant', `Persian$\_$cat'\}, with `Persian$\_$cat' being the true label. All three classes are quite dissimilar from each other. Hence, all OT based loss functions relatively penalize both the incorrect classes similarly.}\label{fig:cwe}
% \end{figure}



% \begin{figure}[t]
% \center
% \includegraphics[width=.5\textwidth]{figs/RboTvsM22_Blue_whale_Dolphin_kl_1e-2.pdf}
% \caption{Contour plots of various OT distance based loss functions. The labels are \{`Blue$\_$whale', `Dolphin', `Humpback$\_$whale'\}, with `Humpback$\_$whale' as the true label. All three classes share similar characteristics but `Blue$\_$whale is more similar to `Humpback$\_$whale'.}\label{fig:llt}
% \end{figure}

\subsection{Multi-label learning with the ${\rm W}_{\rm ROT}$ loss}
We propose to employ the robust OT distance-based loss in multi-label/multi-class problems. To this end, we solve the empirical risk minimization problem, i.e.,
\begin{equation}\label{eqn:multi-label}
    \minop_{\bW\in\R^{M\times L}}\ \frac{1}{N} \sum_{j=1}^N{\rm W}_{\rm ROT}(h(\bx_j;\bW),\hat{\by}_j),
\end{equation}
where ${\rm W}_{\rm ROT}$ is the robust OT distance-based function  (\ref{eqn:MahalanobisRobustOT}). Here, ${\rm W}_{\rm ROT}$ may be set to any of the discussed robust OT distance functions such as ${\rm W}_{\rm P}$ (\ref{eqn:proposed-p-norm-min}), ${\rm W}_{\rm KL}$ (\ref{eqn:proposed-min-kl-divergence}), and ${\rm W}_{\rm DS}$ (\ref{eqn:proposed-doubly-stochastic}). As discussed, \cite{frogner15a} employs ${\rm W}_p^p(h(\bx;\bW),\hat{\by})$ as the loss function in (\ref{eqn:multi-label}).

In Figure~\ref{fig:cce}, we analyze the nature of the ${\rm W}_2^2$-based loss function and the proposed ${\rm W}_{\rm ROT}$-based loss functions by viewing their contours plots for a three-class setting with labels as \{`Siamese$\_$cat', `Elephant', `Persian$\_$cat'\}. We consider label `Persian$\_$cat' as true label, i.e., $\hat{\by}=[0,0,1]^\top$, and consider predictions of the form $\bh=[x,y,1-x-y]$. The ground cost function is computed using the fastText word embeddings corresponding to the labels \cite{bojanowski16a}. All the plots are made to same scale by normalizing the highest value of the loss to $1$. The first and the third classes in this setting are similar, and the OT distance based loss functions should exploit this relationship via the ground cost function. We observe that all the four losses in Figure~\ref{fig:cce} penalize `Elephant' more than `Siamese$\_$cat'. However, the contours of ${\rm W}_2^2$ loss in  Figure~\ref{fig:cce}(a) are linear, while those of the proposed ${\rm W}_{\rm P}$ with $k=1$ Figure~\ref{fig:cce}(b) are elliptical. On the other hand, the proposed ${\rm W}_{\rm KL}$ and ${\rm W}_{\rm DS}$ exhibit varying degree of non-linear contours. 
Overall, the proposed robust OT distance based loss functions enjoy more flexibility in the degree of penalization than the ${\rm W}_2^2$ loss, which may be helpful in certain settings. 

%We analyze the nature of the ${\rm W}_2^2$-based loss function and the proposed ${\rm W}_{\rm ROT}$-based loss functions by viewing their contours plots for a three-class setting with labels as \{\textit{A},\textit{B},\textit{C}\}. We consider label \textit{C} as true label, i.e., $\hat{\by}=[0,0,1]^\top$, where the first dimension corresponds to label \textit{A} and consider predictions of the form $\bh=[a,b,1-a-b]$. Since $h$ is obtained from the softmax function (\ref{eqn:softmax}), we have $(a,b) \in \{(x,y):0\leq x,y\leq 1 {\rm \ and \ }x+y\leq 1\}$. The ground cost function is computed using the fastText word embeddings corresponding to the labels \cite{bojanowski16a}. We plot the contour maps of ${\rm W}_2^2(\bh,\hat{\by})$ and the proposed ${\rm W}_{\rm P}(\bh,\hat{\by})$, ${\rm W}_{\rm KL}(\bh,\hat{\by})$, and ${\rm W}_{\rm DS}(\bh,\hat{\by})$, as $(a,b)$ varies along the two-dimensional $X-Y$ plane. All the plots are made to same scale by normalizing the highest value of the loss to $1$.

%In Figure~\ref{fig:cce}, we consider the labels as \{\textit{A},\textit{B},\textit{C}\}=\{`Siamese$\_$cat', `Elephant', `Persian$\_$cat'\}. The first and the third classes in this setting are similar, and the OT distance based loss functions should exploit this relationship via the ground cost function. With `Persian$\_$cat' as the true class, we observe that all the four losses in Figure~\ref{fig:cce} penalize `Elephant' more than `Siamese$\_$cat'. However, the contours of ${\rm W}_2^2$ loss in  Figure~\ref{fig:cce}(a) are linear, while those of the proposed ${\rm W}_{\rm P}$ with $k=1$ Figure~\ref{fig:cce}(b) are elliptical. On the other hand, the proposed ${\rm W}_{\rm KL}$ and ${\rm W}_{\rm DS}$ exhibit varying degree of non-linear contours. Overall, the proposed robust OT distance based loss functions enjoy more flexibility in the degree of penalization than the ${\rm W}_2^2$ loss, which may be helpful in certain learning settings. 
%is reflected by their better empirical performance (Section~\ref{sec:experiments}) in discriminative learning setting.
%Overall, the proposed robust OT distance based loss functions penalize 'Siamese$\_$cat' relatively lesser than the ${\rm W}_2^2$ loss, implying a better discriminative behavior.

% In Figure~\ref{fig:cwe}, we consider the labels as \{\textit{A},\textit{B},\textit{C}\}=\{'Blue$\_$cat', 'Elephant', 'Persian$\_$cat'\}. The two classes `Blue$\_$cat' and `Elephant' are quite dissimilar to the true class `Persian$\_$cat'. We observe that while the ${\rm W}_2^2$ loss exhibits similar linear contours as previously (but with a different slope),  non-linearity in the proposed robust OT based losses allow them more freedom to adapt. 
% We provide contour maps for another interesting setting, where all the three classes are similar, but one class is more closer to the true class. In Figure~\ref{fig:llt}, we consider the labels as \{\textit{A},\textit{B},\textit{C}\}=\{'Blue$\_$whale', 'Dolphin', 'Humpback$\_$whale'\}.







\subsection{Optimizing ${\rm W}_{\rm ROT}$ loss}

We solve Problem (\ref{eqn:multi-label}) using the standard stochastic gradient descent (SGD) algorithm. In each iteration of the SGD algorithm, we pick a training instance $j = \{1, \ldots, N \}$ and update the parameter $\bW$ along the negative of the gradient of the loss term ${\rm W}_{\rm ROT}(h(\bx_j;\bW),\hat{\by}_j))$ with respect to the model parameter $\bW$. 

We obtain it using the chain rule by computing $\nabla_\bW h(\bx_j;\bW)$ and $\nabla_{h(\bx;\bW)} {\rm W}_{\rm ROT}(h(\bx_j;\bW),\hat{\by}_j)$. While the expression for $\nabla_\bW h(\bx_j;\bW)$ is well studied, computing $\nabla_{h(\bx;\bW)} {\rm W}_{\rm ROT}(h(\bx_j;\bW),\hat{\by}_j)$ is non trivial as the loss ${\rm W}_{\rm ROT}(h(\bx_j;\bW),\hat{\by}_j)$ involves a min-max optimization problem  (\ref{eqn:MahalanobisRobustOT}). To this end, we consider a regularized version of ${\rm W}_{\rm ROT}$ by adding a negative entropy regularization term to (\ref{eqn:fgamma}). Equivalently, we consider the formulation for computing the robust OT distance between $h(\bx_j;
\bW)$ and $\hat{\by}_j$ as
\begin{equation}\label{eqn:rotminmax}
\begin{array}{ll}
  {\rm W}_{\rm ROT}(h(\bx_j;\bW),\hat{\by}_j) = \\
  \minop_{\gamma \in \Pi(h(\bx_j;\bW),\hat{\by}_j)} \maxop_{\bM \in \calM} \inner{\bV_\gamma,\bM} \\
  \qquad \qquad \qquad \qquad \qquad + \lambda_{\gamma} \sum_{pq} \gamma_{pq} {\rm ln}(\gamma_{pq}),
  \end{array}
\end{equation}
where $\lambda_{\gamma} >0$ and $\bV_{\gamma} = \sum_{pq} (\bl_p - \bl_q)(\bl_p - \bl_q)^\top \gamma_{pq}$ is of size $d \times d$. Here, $\bl_p$ is the ground embedding of $p$-th label of dimension $d$. We next provide an expression for the gradient of ${\rm W}_{\rm ROT}(h(\bx_j;\bW),\hat{\by}_j)$ with respect to $h(\bx; \bW)$.

\begin{Lem}\label{lemma:gradient_rot}
Let $(\gamma^{*}, \bM^*(\gamma^*))$ denote the optimal solution of the robust OT problem (\ref{eqn:rotminmax}). Then, 
\begin{equation}\label{eqn:gradient_rot}
\begin{array}{lll}
\nabla_{h(\bx;\bW)} {\rm W}_{\rm ROT}(h(\bx_j;\bW),\hat{\by}_j) =  \frac{1}{L}\bA \bone - \frac{\bone ^\top \bA \bone}{L^2} \bone,
\end{array}
\end{equation}
where $\bone $ is the column vector of ones of size $L$, $\bA = \bC^*+ \lambda_{\gamma } ({\rm ln}(\gamma ^*) + \bone \bone^\top)$, and $\bC^*(\bl_p,\bl_q) = (\bl_p - \bl_q)^\top \bM^*(\gamma^*) (\bl_p - \bl_q)$ is of size $L \times L$.
\end{Lem}
% \begin{proof}
% The proof is in Appendix \ref{supp:sec:proof_gradient_rot}.
% \end{proof}

For the multi-label setting, computation of the gradient $\nabla_{h(\bx;\bW)} {\rm W}_{\rm ROT}(h(\bx_j;\bW),\hat{\by}_j)$, shown in (\ref{eqn:gradient_rot}), in Lemma \ref{lemma:gradient_rot} costs $O(l_j Ld^2)$, where $l_j$ is the number of ground-truth labels for the $j$-th training instance. Using the modeling (\ref{eqn:factorizeMahalanobis}), the cost reduces to $O(l_jLr^2)$. In many cases, $l_j$ is much smaller than $L$. In the multi-class setting, the gradient computation cost reduces to costs $O(Ld^2)$ by setting $l_j = 1$. 
Using the modeling (\ref{eqn:factorizeMahalanobis}), it can be reduced to $O(Lr^2)$. 

Overall, in both multi-class/multi-label settings, the cost of the gradient computation in (\ref{eqn:gradient_rot}) scales linearly with the number of labels $L$ and quadratically with $r$. When $r \ll d$, optimization of the ${\rm W}_{\rm ROT}$ loss becomes computationally feasible for large-scale multi-class/multi-label instances.








\section{Experiments}\label{sec:experiments}
We evaluate the proposed robust optimal transport formulations in the supervised multi-class/multi-label setting discussed in Section~\ref{sec:ROTloss}. Our code is available at \url{https://github.com/satyadevntv/ROT4C}. 



% \begin{figure}[t]
% \center
% \includegraphics[width=.45\textwidth]{figs/mAP_v_epoch.pdf}
% \caption{Evolution of mean average precision (mAP) on the Flickr tag-prediction dataset for various OT distance-based loss functions.}\label{fig:flickr}
% \end{figure}





\subsection{Datasets and evaluation setup}
We experiment on the following three multi-class/multi-label datasets. 

\textbf{Animals} \cite{lampert13a}: This contains $30\,475$ images of $50$ different animals. We employed $4096$ dimensional DeCAF features. 
%DeCAF features ($4096$ dimensions) of each image are available at \url{https://github.com/jindongwang/transferlearning/blob/master/data/dataset.md}. We randomly sample $10$ samples per class for training and the rest are used for evaluation.




\textbf{MNIST}: The MNIST handwritten digit dataset consists of $28\times 28$ dimensional images of digits $\{0,\ldots,9\}$. 
%The images are of $28\times 28$ pixels, leading to $784$ features. The pixel values are normalized by dividing each dimension with $255$. We randomly sample $100$ images per class (digit) for training and $1000$ images per class for evaluation.

\textbf{Flickr} \cite{thomee16a}: The Yahoo/Flickr Creative Commons 100M dataset  consists of descriptive tags for around 100M images. We follow the experimental protocol in \cite{frogner15a} for the tag-prediction (multi-label) problem on $1000$ descriptive tags. 
%The training and test sets consist of $10\,000$ randomly selected images associated with these tags. 
%The features for images are extracted using MatConvNet \cite{vedaldi15a}. 
%The train/test sets as well as the image features are available at \url{http://cbcl.mit.edu/wasserstein}. 


\begin{table}[t]
  \caption{Performance of various OT distance based loss functions}\label{table:results}
%   \begin{center}
    \begin{tabular}{lccccc}
      \toprule
      \multirow{2}{*}{Loss} & \multirow{2}{*}{$r$} & Animals & MNIST & \multicolumn{2}{c}{Flickr} \\ 
      & & (AUC) & (AUC) & (AUC) & (mAP) \\
      \midrule
      \multirow{1}{*}{${\rm W}_2^2$} \cite{frogner15a} & $-$ & $0.794$ & $0.848$ & $0.649$ & $0.0209$\\
      \addlinespace[0.3em]
      \multirow{1}{*}{${\rm SRW}_2^2$} \cite{paty19a} & $-$ & $0.802$ & $0.925$ & $0.734$ & $0.0370$\\
      \addlinespace[0.3em]
      \multirow{1}{*}{${\rm SRW}_5^2$} \cite{paty19a} & $-$ & $0.855$ & $0.860$ & $0.730$ & $0.0360$\\
      \addlinespace[0.3em]
      \multirow{1}{*}{${\rm SRW}_{10}^2$} \cite{paty19a} & $-$ & $0.860$ & $0.788$ & $0.721$ & $0.0350$\\
      \addlinespace[0.3em]
      \multirow{1}{*}{${\rm SRW}_{20}^2$} \cite{paty19a} & $-$ & $0.850$ & $0.788$ & $0.719$ & $0.0352$\\
      \addlinespace[0.3em]
      \multirow{1}{*}{${\rm RKP}_{4/3}$} \cite{dhouib20a} & $-$ & $0.854$ & $0.914$ & $0.732$ & $0.0366$\\
      \addlinespace[0.3em]
      \multirow{1}{*}{${\rm RKP}_{4}$} \cite{dhouib20a} & $-$ & $0.850$ & $0.860$ & $0.709$ & $0.0350$\\
      \addlinespace[0.3em]
      \multirow{1}{*}{${\rm RKP}_{\infty}$} \cite{dhouib20a} & $-$ & $0.837$ & $0.921$ & $0.735$ & $0.0370$\\
      \midrule
      \multirow{3}{*}{${\rm W_{P}}$, $k=1$  (Eq.~\ref{eqn:proposed-p-norm-min})} & $5$ & $0.801$ & $\mathbf{0.959}$ & $0.706$ & $0.0481$\\
      & $10$ & $0.907$ & $0.940$ & $0.745$  & $0.0625$\\
      & $20$ & $\mathbf{0.908}$ & $0.922$ & $\mathbf{0.768}$  & $\mathbf{0.0717}$\\
      \midrule
      \multirow{3}{*}{${\rm W_{P}}$, $k=2$ (Eq.~\ref{eqn:proposed-p-norm-min})} & $5$ & $0.890$ & $0.804$ & $0.760$  & $0.0625$\\
      & $10$ & $0.878$ & $0.702$ & $0.742$  & $0.0468$\\
      & $20$ & $0.874$ & $0.603$ & $0.737$  & $0.0441$\\
      \midrule
      \multirow{3}{*}{${\rm W_{KL}}$ (Eq.~\ref{eqn:proposed-min-kl-divergence})} & $5$ & $0.794$ & $0.867$ & $0.648$  & $0.0207$\\
      & $10$ & $0.749$ & $0.870$ & $0.649$  & $0.0205$\\
      & $20$ & $0.794$ & $0.779$ & $0.649$  & $0.0205$\\
      \midrule
      \multirow{3}{*}{${\rm W_{DS}}$ (Eq.~\ref{eqn:proposed-doubly-stochastic})} & $5$ & $\mathbf{0.908}$ & $0.927$ & $0.724$  & $0.0530$\\
      & $10$ & $0.878$ & $0.873$ & $0.668$  & $0.0325$\\
      & $20$ & $0.845$ & $0.813$ & $0.628$  & $0.0219$\\
      \bottomrule
    \end{tabular}
%   \end{center}
\end{table}

\textbf{Experimental setup and baselines}: As described in Section~\ref{sec:ROTloss}, we use the fastText word embeddings \cite{bojanowski16a} corresponding to the labels for computing the OT ground metric in all our evaluations. 
We report the standard AUC metric for all the experiments. For the Flickr tag-prediction problem, we additionally report the mAP (mean average precision) metric. As the datasets are high dimensional, we use the low-dimensional modeling of the Mahalanobis metric $\bM$ (Section~\ref{sec:low_dimensional_metric_decomposition}) for the proposed robust OT distance-based loss functions by randomly grouping the features. We experiment with $r\in\{5,10,20\}$. 
%As baseline, we report the results with the ${\rm W}_2^2$ distance-based loss function (\ref{eqn:W22distance}) on all the datasets. 
In addition to the proposed robust OT distances (Section~\ref{sec:formulations}), we report results with the following OT distance-based loss functions as baselines:
\begin{itemize}
    \item ${\rm W}_2^2$: the $2$-Wasserstein distance (\ref{eqn:W22distance}).
    \item ${{\rm SRW}}_k^2$: the subspace robust Wasserstein distance (\ref{eqn:SRW1}) proposed by Paty et al.~\cite{paty19a}. We obtain results for several hyper-parameter values $k=\{2,5,10,20\}$.
    \item ${\rm RKP}_\rho$: this class of robust Wasserstein distances \cite{dhouib20a} is parameterized by the Schatten $\rho$-norm regularized Mahalanobis metric. We obtain results for several hyper-parameter values $\rho=\{4/3,4,\infty\}$. As shown in \cite{dhouib20a}, ${\rm RKP}_1={\rm W}_2^2$ and ${\rm RKP}_\infty={{\rm SRW}}_1^2$. 
\end{itemize}
Our experiments are run on a machine with 32 core Intel CPU ($2.1$ GHz Xeon) and a single NVIDIA GeForce RTX 2080 Ti GPU ($11$ GB). 
The model computations for all algorithms on all datasets are performed on the GPU, except on Flickr where the baselines ${\rm RKP}_\rho$ and ${{\rm SRW}}_k^2$ have only CPU-based implementation. This is because the memory requirement for ${\rm RKP}_\rho$ and ${{\rm SRW}}_k^2$ on Flickr is too large for our GPU. 
The low-dimensional modeling for the proposed robust OT distances (with $r\ll d$) in Section~\ref{sec:low_dimensional_metric_decomposition} makes GPU implementation feasible on all datasets for ${\rm W_{P}}$, ${\rm W_{KL}}$, and ${\rm W_{DS}}$. Additional experimental details are in \cite{jawanpuria20a}.




\begin{figure}[t]
\center
\includegraphics[width=.35\textwidth]{draft/figs/flickr_timings_notype3.pdf}
\caption{Time taken per epoch versus $r$ on the Flickr dataset by our algorithm with the proposed ${\rm W}_{\rm P}$ loss with $k=1$.}\label{fig:timing}
\end{figure}






\subsection{Results and discussion}

\textbf{Generalization performance}: We report the results in Table~\ref{table:results}. Overall, we observe that the proposed robust OT distance based loss functions provide better generalization performance than the considered baselines. We also evaluate the robustness of proposed OT distance-based loss functions with respect to randomized grouping of the features into $r$ groups. As discussed in Section~\ref{sec:low_dimensional_metric_decomposition}, the low-dimensional modeling of $\bM$ requires dividing the $d$ features into $r$ groups. Results on the proposed robust OT distance in Table~\ref{table:results} are obtained by one randomized grouping of features. In \cite{jawanpuria20a}, we report the mean AUC and the corresponding standard deviation obtained across five random groupings of features on the same train-test split (for the smaller Animals and MNIST datasets). We observe that the results across various randomized feature groupings is quite stable, signifying the robustness of the proposed OT distance-based loss functions with regards to groupings of features.


%The proposed ${\rm W}_{\rm P}$ loss with $k=1$ obtains the best results on all the three datasets. 
%The proposed ${\rm W}_{\rm P}$ loss with $k=2$ obtains a good AUC/mAP on the Animals and the Flickr datasets but does not generalize well in MNIST. Similarly, while ${\rm W}_{\rm DS}$ with $r=5$ obtains good results, its performance decreases with $r$. This is because the non-linear nature of the proposed OT distance-based loss function may lead to overfitting, especially at high $r$. 

\textbf{Computation timing}: We also report the time taken per epoch of the SGD algorithm on the Flickr dataset with ${\rm W}_{\rm P}$ $(k=1)$ as the loss function. From Figure~\ref{fig:timing}, we observe that our model scales gracefully as $O(r^2)$ as discussed in Section~\ref{sec:algorithms}. %Empirically, we show that we can obtain a good generalization performance and computational efficiency with $r\ll d$. 
We next compare per-epoch time take by our ${\rm W_{P}}$ loss with $r=20$ against those taken by the robust OT baselines ${{\rm SRW}}_k^2$ and ${\rm RKP}_\rho$. The per-epoch time taken by ${{\rm SRW}}_k^2$ and ${\rm RKP}_\rho$ is $14$-$16$s for Animals, $23$-$26$s for MNIST, and around $12.5$ hours for Flickr. The per-epoch time taken by our W$_{\rm P}$ loss with $r=20$ is $0.3$s (Animals), $0.5$s (MNIST), and $87.5$s (Flickr). Hence, on Animals and MNIST datasets, computing the proposed robust OT distances is at least $45$ times faster than both ${{\rm SRW}}_k^2$ and ${\rm RKP}_\rho$. 
This is due to a) efficient computation of optimal $\bM$ (Section~\ref{sec:formulations}) and b) low-dimensional modeling of $\mathbf{M}$ (Section~\ref{sec:low_dimensional_metric_decomposition}).


\section{Conclusion}
We discussed robust optimal transport problems arising from the Mahalanobis metric parameterized ground cost functions. A particular focus was on discussing novel formulations that may be computed efficiently. We also proposed a low-dimensional modeling of the Mahalanobis metric for efficient computation of robust OT distances. %The parameter $r$ here allows to trade-off accuracy with computational benefit. 
An immediate outcome is that it allows the use the robust OT formulations in high-dimensional multi-class/multi-label settings. Results on real-world datasets demonstrate the efficacy of the proposed robust OT distances in learning problems. 

%\section*{Acknowledgment}
%We thank J. Saketha Nath for insightful discussions. 




==> main_old.tex <==
\begin{abstract}
The problem of robust optimal transport (OT) aims at recovering the best transport plan with respect to the worst possible cost function. In this work, we study novel robust OT formulations where the cost function is parameterized by a symmetric positive semi-definite Mahalanobis metric. In particular, we study several different regularizations on the Mahalanobis metric -- element-wise $p$-norm, KL-divergence, and doubly-stochastic constraint -- and show that the resulting optimization formulations can be considerably simplified by exploiting the problem structure. For large-scale applications, we additionally propose a suitable low-dimensional decomposition of the Mahalanobis metric for the studied robust OT problems. Overall, we view the robust OT (min-max) optimization problems as non-linear OT (minimization) problems, which we solve using a Frank-Wolfe algorithm. We discuss the use of robust OT distance as a loss function in multi-class/multi-label classification problems. Empirical results on several real-world tag prediction and multi-class datasets show the benefit of our modeling approach. 
\end{abstract}
%For several class of regularizations on the metric, e.g.,  element-wise $p$-norm, KL-divergence, or doubly-stochastic constraint, we show that the optimization of the proposed robust OT problem may be considerably simplified by dropping the positive semi-definite constraint on the metric (but still obtaining a globally optimal solution). 

\section{Introduction}\label{sec:intro}
Optimal transport \citep{peyre19a} has become a popular tool in diverse machine learning applications such as domain adaptation \citep{courty17a}, multi-task learning \citep{janati19a}, natural language processing \citep{melis18a}, computer vision \citep{rubner00}, classification \citep{frogner15a}, generative model training \citep{genevay18a,arjovsky17a}, to name a few. 
The optimal transport (OT) metric between two probability measures, also known as the Wasserstein distance or the earth mover's distance (EMD), defines a geometry over the space of probability measures \citep{villani09a} and evaluates the minimal amount of work required to transform one measure into another with respect to the ground cost function. 

Given two probability measures $\mu_1$ and $\mu_2$ over metric spaces $\calS$ and $\calT$, respectively, the optimal transport problem due to \citet{kantorovich42a} aims at finding a transport plan $\gamma$ as a solution to the following problem:
\begin{equation}\label{eqn:optimal-transport}
    {\rm W}_c(\mu_1,\mu_2) = \inf_{\gamma\in\Pi(\mu_1,\mu_2)} \int_{\calS\times\calT} c(\bs,\bt) d\gamma(\bs,\bt),
\end{equation}
where $\Pi(\mu_1,\mu_2)$ is the set of joint distributions with marginals $\mu_1$ and $\mu_2$ and $c:\calS \times \calT \rightarrow \R_{+}:(\bs,\bt)\rightarrow c(\bs,\bt)$ represents the transportation cost function. We obtain the popular $2$-Wasserstein distance by setting the cost function as the squared Euclidean function, i.e.,  $c(\bs,\bt)=\norm{\bs-\bt}^2$ when $\bs,\bt\in\R^d$. The $2$-Wasserstein distance can be reformulated as follows \citep{paty19a}:
\begin{equation}\label{eqn:W22distance}
    {{\rm W}}_2^2(\mu_1,\mu_2) = \minop_{\gamma\in\Pi(\mu_1,\mu_2)} \inner{\bV_\gamma,\bI},
\end{equation}
where $\bV_\gamma\coloneqq\int_{\calS\times\calT} (\bs-\bt)(\bs-\bt)^\top d\gamma(\bs,\bt)$ and $\bI$ is the identity matrix. 

% The optimal transport between discrete probability measures $\mu_1$ and $\mu_2$ may be formulated as the following optimization problem \citep{kantorovich42a}: 
% \begin{equation}\label{eqn:optimal-transport}
% {\rm W}_c(\mu_1,\mu_2) = \min_{\gamma\in\Pi(\mu_1,\mu_2)} \inner{\gamma,\bC},
% \end{equation}
% where $\bC\in\R_{+}^{m\times n}$ is a ground cost matrix, $\mu_1\in\Delta_m$, $\mu_2\in\Delta_n$, $\Delta_m\coloneqq\{\bw\R^{m}:\bw\geq\bzero;\bw^\top=1\}$, and $\Pi(\mu_1,\mu_2)$ is the set of joint probability distribution with marginals $\mu_1$ and $\mu_2$, i.e., $\Pi(\mu_1,\mu_2)=\{\gamma\in\R^{m\times n}:\gamma\geq \bzero;\gamma \bone=\mu_1;\gamma^\top\bone=\mu_2\}$. 

% between the source distribution's samples  $\bX=\{\bx_i\}_{i=1}^m\in\R^{d\times m}$ and the target distribution's samples $\bY=\{\by_i\}_{i=1}^n\in\R^{d\times n}$, the $(i,j)$-th entry of $\bC$ is $c(\bx_i,\by_j)$, $c(\bx,\by)$ is the given ground cost function, $\mu_1$ and $\mu_2$ are the given discrete source and target distributions, respectively, and $\Pi(\mu_1,\mu_2)$ is the set of feasible joint transportation plan: $\Pi(\mu_1,\mu_2)=\{\gamma\in\R^{m\times n}:\gamma\geq \bzero;\gamma \bone=\mu_1;\gamma^\top\bone=\mu_2\}$. 
% The special case of $c(\bx,\by)=\norm{\bx-\by}^2$ (squared Euclidean distance) is popularly denoted by ${{\rm W}}_2^2$ (the $2$-Wasserstein distance) and can be reformulated as follows \citep{paty19a}: 
% %$ {{\rm W}}_2^2(\mu_1,\mu_2) = \min_{\gamma\in\Pi(\mu_1,\mu_2)}\ \inner{\bV_\gamma,\bI}$, 
% \begin{equation}\label{eqn:W22distance}
%     {{\rm W}}_2^2(\mu_1,\mu_2) = \minop_{\gamma\in\Pi(\mu_1,\mu_2)}\ \inner{\bV_\gamma,\bI},\\
%     %&=& \minop_{\gamma\in\Pi(\mu_1,\mu_2)} \trace(\bV_\gamma),
% \end{equation}
% where $\bV_\gamma=\sum_{ij} (\bx_i-\by_j)(\bx_i-\by_j)^\top \gamma_{ij}$ and $\bI$ is the identity matrix. 


%\citep{paty19a} proposed a subspace robust variant of the Wasserstein distance that considers the maximal distance between two probability measures when they are projected on a lower dimensional subspace. 
%More generally, 



\subsection*{Robust optimal transport} 

Recent works \citep{paty19a,kolouri19a,deshpande19a} have proposed variants of the Wasserstein distance that aim at maximizing the OT distance between two probability measures in a projected low-dimensional space, which may be viewed as instances of robust OT distance.
%Such OT distances are typically modeled as \commentPJ{max-min/min-max} optimization problems and may be viewed as instances of the robust OT distance. 
In general, the robust OT distance aims at maximizing the minimal transport cost over a set of ground cost functions.

\citet{paty19a} propose a robust variant of the ${\rm W}_2^2$ distance, termed as the Subspace Robust Wasserstein (SRW) distance, as follows: 
%${{\rm SRW}}_k^2(\mu_1,\mu_2) = \max_{\bM\in\calM}\min_{\gamma\in\Pi(\mu_1,\mu_2)}\ \inner{\bV_\gamma,\bM}$, 
\begin{equation}\label{eqn:SRW1}
%%\begin{array}{lll}
    {{\rm SRW}}_k^2(\mu_1,\mu_2) = \maxop_{\bM\in\calM} \minop_{\gamma\in\Pi(\mu_1,\mu_2)}\ \inner{\bV_\gamma,\bM},\\
%    %&=&\minop_{\gamma\in\Pi(\mu_1,\mu_2)} \sum\limits_{i=1}^k \lambda_i(\bV_\gamma),
%%\end{array}
\end{equation}
where the domain $\calM$ is defined as $\calM=\{\bM:\bzero\preceq\bM\preceq\bI {\rm \ and \ } \trace(\bM)=k\}$. 
It should be noted that $\inner{\bV_\gamma,\bM}=\int_{\calS\times\calT} c_\bM(\bs,\bt) d\gamma(\bs,\bt)$, where $c_{\bM}(\bs,\bt)=(\bs-\bt)^\top\bM(\bs-\bt)$ is a cost function parameterized by a symmetric positive semi-definite matrix or a Mahalanobis metric $\bM$ of size $d\times d$. 
%It should be noted that $\inner{\bV_\gamma,\bM}=\sum_{i,j}\gamma_{ij}c_{\bM}(\bx_i,\by_j)$, where $c_{\bM}(\bx,\by)=(\bx-\by)^\top\bM(\bx-\by)$ is a Mahalanobis metric parameterized cost function. 


\citet{dhouib20a} also study the form (\ref{eqn:SRW1}) of Mahalanobis metric parameterized cost functions in the robust OT setting, but with the domain $\calM$ defined as $\calM=\{\bM:\bM\succeq\bzero {\rm \ and\ } \norm{\bM}_{*p}=1\}$, where $\norm{\cdot}_{*p}$ denotes the Schatten $p$-norm regularizer, i.e., $\norm{\bM}_{*p}\coloneqq(\sum_i \sigma_i(\bM)^p)^\frac{1}{p}$. Here, $\sigma_i(\bM)$ denotes the $i$-th largest eigenvalue of $\bM$. 

Both \citep{paty19a,dhouib20a} pose their Mahalanobis metric parameterized robust optimal transport problems as optimization problems over the metric $\bM$. This involves satisfying the positive semi-definite constraint at every iteration, which typically requires costly eigenvalue decomposition operations costing $O(d^3)$. 


\subsection*{Contributions}
In this paper, we focus on the robust OT distance formulations arising from Mahalanobis metric parameterized cost functions and discuss several novel regularizations and algorithmic approaches to use them in learning problems. Our main contributions are the following.


\begin{itemize}
\item We discuss three families of regularizers on $\bM$:  entry-wise $p$-norm for $p\in(1,2]$, KL-divergence based regularization, and the doubly-stochastic regularization. We show that for those regularizers, enforcement of the symmetric positive semi-definite constraint is not needed as the problem structure {\it implicitly} learns a symmetric positive semi-definite matrix at optimality. The implications are two fold. First, the computational cost of computing the robust OT distance is $O(d^2)$ as against $O(d^3)$ (when using the existing regularizers). Second, our optimization methodology for computing the robust OT distance simplifies. 

\item To further reduce the computational burden of the robust OT distance computation, we propose a novel $r$-dimensional decomposition of the Mahalanobis metric for the studied robust OT
problems, resulting in the per-iteration computational cost of $O(r^2)$, where $r \ll d$. The parameter $r$ provides an effective trade-off between computational efficiency and accuracy. 

\item We discuss how to use the robust distance as a loss in multi-class/multi-label classification problems. 

\end{itemize}


The outline of the paper is as follows. Section \ref{sec:formulations} discusses the proposed regularizations. The novel decomposition of the metric is discussed in Section \ref{sec:low_dimensional_metric_decomposition}. We formulate the robust OT distance problem as a non-linear OT (minimization) problem in $\gamma$. In Section \ref{sec:algorithms}, this interpretation allows to develop a Frank-Wolfe algorithm. The setup of using the robust OT distance in learning problems is discussed in Section \ref{sec:ROTloss}. In Section \ref{sec:experiments}, we show the good performance of our modeling approach in several real-world prediction datasets: Animals with attributes, MNIST, and Flickr. 

%All proofs and additional experimental details are supplied as supplementary material.

%\commentPJ{We can give outline of the paper here and also write about all proofs in the supplementary material.}


















%When $\CC$ is a convex set, robust OT distance may also be modeled via a min-max objective which has the following interpretations: recover the best transport plan with respect to the worst possible ground cost function \citep{dhouib20a}.  
%Robust OT problems have been explored for robustness to noise in high dimensional data \citep{paty19a}, for submodular cost functions. 
%Computing them typically requires solving a a min-max (or a max-min) optimization problem.




% The main contributions of this work are as follows:
% \begin{itemize}
%     \item we propose novel robust OT formulations where the cost function is parameterized by the Mahalanobis metric $\bM\succeq\bzero$. For the proposed families of regularizers on $\bM$, we show that the problem may be solved by dropping the positive semi-definiteness constraint on metric $\bM$ ($\bM\succeq\bzero$) as the resulting optimal solution $\bM^{*}$ satisfies $\bM^{*}\succeq\bzero$. This considerably simplifies our optimization methodology. The proposed family of regularizers on the Mahalanobis metric $\bM$ include entry-wise $p$-norm for $p\in(1,2]$, KL-divergence based regularization, and the doubly stochastic regularization. 
%     \item we develop two approaches for solving the proposed robust OT formulations. The first is a Frank-Wolfe algorithm which requires regularization on the transport plan \citep{cuturi13a} for efficiency. Our second approach employs the Riemannian optimization framework and does not require additional regularization on the transport plan. We propose efficient first- and second-order Riemannian algorithms for the robust OT problems. 
%     \item \commentPJ{Empirical contributions}
% \end{itemize}

% We study robust optimal transport problems of the form:
% \begin{equation}\label{eqn:RKP}
% {\rm RKP}(\Pi,\CC) = \max_{c\in\CC}\min_{\gamma\in\Pi}  \sum\limits_{i,j}\gamma_{ij}c(\bx_i,\by_j),
% \end{equation}
% where $c(\bx,\by)$ is the cost of moving $\bx$ to $\by$ (drawn from distributions $\mu_1$ and $\mu_2$, respectively). Overall, (\ref{eqn:RKP}) aims at learning a cost function, which maximizes the minimium Wasserstein distance between a given pair of distributions. In this work, we study efficient formulations and algorithms for (\ref{eqn:RKP}) when $\CC$ is a convex set. 








% \subsection{Background}
% The optimal transport (OT) problem may be formulated as:
% \begin{equation}\label{eqn:optimal-transport}
% \gamma^{*} \coloneqq \argmin_{\gamma\in\Pi(\mu_1,\mu_2)} \inner{\gamma,\bC}_F,
% \end{equation}
% where $\bC$ is the given cost matrix. The special case of employing the squared Euclidean distance as the cost, popularly denoted by ${{\rm W}}_2^2$ ($2$-Wasserstein distance), is as follows: 
% \begin{equation}\label{eqn:W22distance}
% %\begin{array}{lll}
%     {{\rm W}}_2^2(\mu_1,\mu_2) = \minop_{\gamma\in\Pi(\mu_1,\mu_2)}\ \inner{\bV_\gamma,\bI},\\
%     %&=& \minop_{\gamma\in\Pi(\mu_1,\mu_2)} \trace(\bV_\gamma),
% %\end{array}
% \end{equation}
% where $\bV_\gamma=\sum_{ij} (\bx_i-\by_j)(\bx_i-\by_j)^\top \gamma_{ij}$ and $\bI$ is the identity matrix. 
% \citep{paty19a} propose a robust variant of the $W_2^2$ distance, termed as the Subspace Robust Wasserstein (SRW) distance, as follows:
% \begin{equation}\label{eqn:SRW1}
% %\begin{array}{lll}
%     {{\rm SRW}}_k^2(\mu_1,\mu_2) = \maxop_{\bM\in\calM} \minop_{\gamma\in\Pi(\mu_1,\mu_2)}\ \inner{\bV_\gamma,\bM},\\
%     %&=&\minop_{\gamma\in\Pi(\mu_1,\mu_2)} \sum\limits_{i=1}^k \lambda_i(\bV_\gamma),
% %\end{array}
% \end{equation}
% where the domain $\calM$ is defined as $\calM=\{\bM:\bzero\preceq\bM\preceq\bI; \trace(\bM)=k\}$. 
% It should be noted that $\inner{\bV_\gamma,\bM}=\sum_{i,j}\gamma_{ij}(\bx_i-\by_j)^\top\bM(\bx_i-\by_j)$. 
% Thus, ${{\rm SRW}}_k^2$ learns a worst-case OT cost function  $c_{\bM}(\bx,\by)=(\bx-\by)^\top\bM(\bx-\by)$, which is parameterized by a Mahalanobis metric. 

%The trace regularization in (\ref{eqn:SRW1}) encourages $\bM$ to be of low-rank for $k<d$. It is evident that the SRW distance is an instance of the robust Kantorovich problem (\ref{eqn:RKP}). 
% \begin{equation}\label{eqn:RKP}
% {\rm RKP}(\Pi,\CC) = \min_{\gamma\in\Pi} \max_{c\in\CC} \sum\limits_{i,j}\gamma_{ij}c(\bx_i,\by_j),
% \end{equation}
% where $c(\bx,\by)$ is the cost of moving $\bx$ to $\by$ (drawn from distributions $\mu_1$ and $\mu_2$, respectively). Overall, (\ref{eqn:RKP}) aims at learning a transport plan $\gamma^{*}$ which is robust to the choice of a cost function $c\in\CC$ (best worst achievable transportation cost). 

% Recently, \citep{dhouib20a} study the above form of Mahalanobis metric parameterized cost functions in the robust OT setting, but with the domain $\calM$ defined as $\calM=\{\bM:\bM\succeq\bzero; \norm{\bM}_{*p}=1\}$, where $\norm{\cdot}_{*p}$ denotes the Schatten $p$-norm regularizer, i.e., $\norm{\bM}_{*p}\coloneqq(\sum_i \sigma_i(\bM)^p)^\frac{1}{p}$. Here,   $\sigma_i(\bM)$ denotes the $i$-th largest eigenvalue of $\bM$. 
% They show that this family of regularization include, as special cases, the $W_2^2$ distance with $p=\infty$ (spectral norm) and the $S_1^2$ distance with $p=1$ (trace norm). 

%It should be noted that $p=1$ Schatten norm (the nuclear/trace norm) regularizes the sum of eigenvalues whereas $p=\infty$ Schatten norm (the spectral norm) regularizes the maximum eigenvalue. 


%$\CC_1=\{c^\bM: (\bx,\by)\mapsto (\bx-\by)^\top\bM(\bx-\by);\bM\succeq\bzero,\norm{\bM}_p\leq1\},$
%They show that ${\rm RKP}(\Pi,\CC)=W_2^2(\mu_1,\mu_2)$ with $p=\infty$ and ${\rm RKP}(\Pi,\CC)$ also simplifies to SRW distance \citep{paty19a} with truncated Schatten $p$-norm. The special case of $p=2$ is also discussed in some detail. However, their main contribution is to propose a cutting-set algorithm for solving the general ${\rm RKP}(\Pi,\CC)$ in the discrete case and $\CC$ is an arbitrary convex set of cost matrices with entries $\bC_{ij}=c(\bx_i,\by_j)$.  

%Both \citep{paty19a,dhouib20a} pose their Mahalanobis metric parameterized robust optimal transport problems as an optimization over metric $\bM$. This involves satisfying the positive semi-definite constraint, which typically requires costly eigendecomposition operation of a $d\times d$ matrix in each step. Overall, \citet{paty19a} propose  projected super-gradient and Frank-Wolfe methods to compute the SRW distance (\ref{eqn:SRW1}). \citep{dhouib20a}, on the other hand, propose a cutting-set based method \citep{mutapcic09} to optimize over Schatten $p$-norm regularized Mahalanobis metric. 

%Most existing works solve instances of the robust Kantorovich problem (RKP) (\ref{eqn:RKP}) as an optimization problem over the cost function. \citet{paty19a} solve the max-min problem in (\ref{eqn:SRW1}) via the projected super-gradient and Frank-Wolfe algorithms. While solving the max-min problem, the gradient computation requires solving the inner minimization problem (over $\gamma$), which is an unregularized OT problem, which may be made efficient by regularizing the OT problem \citep{cuturi13a}. \citep{dhouib20a} propose a cutting-set method to solve (\ref{eqn:RKP}) in convex setting. 
%They remark that unlike the robust OT algorithms in \citep{paty19a}, the cutting-set method may also work on non-differentiable robust OT problems. 

%{\color{red} Existing works have studied problem (\ref{eqn:MahalanobisRobustOT}) with the domain $\calM$ defined as $\calM=\{\bM:\bM\succeq\bzero; \norm{\bM}_{*p} \leq 1\}$ \citep{dhouib20a} or $\calM=\{\bM:\bzero\preceq\bM\preceq\bI; \trace(\bM)=k\}$ \citep{paty19a}. They solve the max-min formulation where the outer problem involves positive semi-definite constraints, which typically involves costly eigendecomposition operation of $d\times d$ matrix.}

%It should be noted that the SRW distance is a tight convex relaxation of the (non-convex and non-smooth) projection robust Wasserstein (PRW) distance. \citet{lin20a} propose to directly solve for PRW distance in the Riemannian optimization framework. 








\section{Novel formulations for robust optimal transport}\label{sec:formulations}

In this section, we propose novel formulations of the Mahalanobis metric parameterized robust optimal transport problem, which we rewrite as
\begin{equation}\label{eqn:MahalanobisRobustOT}
    {\rm W}_{\rm ROT}(\mu_1,\mu_2)\coloneqq\minop_{\gamma\in\Pi(\mu_1,\mu_2)}\ f(\gamma),
\end{equation}
where the function $f:\R^{m\times n}\rightarrow\R : \gamma \mapsto f(\gamma)$ is defined as 
\begin{equation}\label{eqn:fgamma}
    f(\gamma)\coloneqq\maxop_{\bM\in\calM}\ \inner{\bV_\gamma,\bM}.
\end{equation}
Here, $\calM=\{\bM:\bM\succeq\bzero {\rm \ and \ }\Omega(\bM) \leq 1\}$ and $\Omega(\cdot)$ is a convex regularizer on the set of positive semi-definite matrices. 
%$\Omega(\cdot)$ may also be an indicator function \commentPJ{(or an indicator function of convex sets)}. 
It should be noted that (\ref{eqn:MahalanobisRobustOT}) is a convex optimization problem. Moreover, by the application of Sion-Kakutani min-max theorem \citep{sion58}, Problem (\ref{eqn:MahalanobisRobustOT}) can be shown to be equivalent to its dual max-min problem:  $\max_{\bM\in\calM}\min_{\gamma\in\Pi(\mu_1,\mu_2)}\inner{\bV_\gamma,\bM}$. 

First-order methods for solving (\ref{eqn:MahalanobisRobustOT}) requires computing the (sub-)gradient $\nabla f(\gamma)$, which can be obtained in terms of an optimal solution $\bM^{*}(\gamma)$ of (\ref{eqn:fgamma}) by using the Danskin's theorem \citep{bertsekas1995nonlinear}. Since (\ref{eqn:fgamma}) involves the positive semi-definite constraint, computing $\bM^{*}(\gamma)$ usually involves costly eigenvalue decomposition (or equivalent operations) of $d\times d$ matrices. However, for the proposed family of regularizers $\Omega(\cdot)$, we show that one can drop the symmetric positive definite constraint in (\ref{eqn:fgamma}) as the optimal solution $\bM^{*}(\gamma)$ of the resulting problem automatically satisfies $\bM^{*}(\gamma) \succeq \bzero$. This considerably simplifies our optimization methodology for the proposed formulations. We discuss the proposed regularizers and the  corresponding $\bM^{*}(\gamma)$ in the following sections. 

%and optimized the following max-min problem:
%\begin{equation}\label{eqn:MahalanobisRobustOTmaxmin}
%     {\rm RKP}(\Pi,\calM) =  \maxop_{\bM\in\calM}\minop_{\gamma\in\Pi(\mu_1,\mu_2)}\ \inner{\bV_\gamma,\bM}.
% \end{equation}

%A key benefit of optimizing the max-min formulation (\ref{eqn:MahalanobisRobustOTmaxmin}) is that the inner problem in $\gamma$ can be solved efficiently via the Sinkhorn-Knopp algorithm by adding the negative entropy regularization \citep{cuturi13a}. Thus, the (sub-)gradient \citep{paty19a} or the linear inequalities corresponding to refinement of the feasible set \citep{dhouib20a} may be computed efficiently. However, the outer optimization problem involves enforcing the positive semi-definite constraints, which typically involves costly eigendecomposition operation of $d\times d$ matrix. 


%Let $\bC$ be a given cost matrix imputed with an unknown noise  $\bN\in\R^{m\times n}$. The noise is assumed to from a family characterized by $\Omega(\bN)\leq 1$, where $\Omega: \R^{m\times n}\rightarrow \R_{+}$ is a regularization function. We begin with the setting when an additive noise influences the cost.

% \textbf{Earth-mover distance (EMD)}: The vanilla OT formulation 
% \begin{equation}\label{eqn:emd}
%  \min_{\gamma\in\Pi}  \inner{\gamma,\hat{\bC}}
% \end{equation}
% may be reformulated in the minimax OT setting by choosing $\Omega(\bN)=\max_{(i,j)}\{\bN_{11},\ldots,\bN_{mn}\}$, i.e., 
% \begin{equation}
%  \min_{\gamma\in\Pi}\ \max_{\bN}\ \inner{\gamma,\hat{\bC}+\bN} - \max_{(i,j)}\{\bN_{11},\ldots,\bN_{mn}\}.
% \end{equation}
% The regularization $\Omega(\bN)\leq 1$ implies that the entries of matrix $\bN$ are upper bounded. 

% \textbf{Sinkhorn distance (dual-Sinkhorn divergence)}: \citet{cuturi13a} introduced the entropy regularization in the optimal transport objective to smoothen the objective and have computational benefits. The resulting distance is termed as the Sinkhorn distance (dual-Sinkhorn divergence), which is computed by solving the following OT problem:
% \begin{equation}\label{eqn:sinkhorn}
%  \min_{\gamma\in\Pi}  \inner{\gamma,\hat{\bC}} + \delta\sum_{ij}\gamma_{ij}\ln{\gamma_{ij}}.
% \end{equation}
% The Sinkhorn distance formulation (\ref{eqn:sinkhorn}) can be equivalently reformulated in the minimax framework (\ref{eqn:minimaxGeneralAdditiveNoise}) by setting $\Omega(\bN)=\delta\ln\left(\sum_{ij}e^{\frac{\bN_{ij}}{\delta}}\right)$, i.e., the log-sum-exp function over the entries of the matrix $\bN$. It should be noted that the log-sum-exp function is a smooth approximation of the maximum function. The latter is employed as the regularizer to reformulate the EMD formulation with the minimax OT framework. 

% \textbf{Element-wise $p$-norm regularization}: \citet{blondel18a} considered the squared $2$-norm regularization over the coupling $\gamma$, with the aim of obtaining truly sparse transportation plan (and which may be computed efficiently). The general squared $p$-norm regularized OT formulation ($p\geq1$) may be written as:
% \begin{equation}\label{eqn:squaredPnorm}
%  \min_{\gamma\in\Pi}  \inner{\gamma,\hat{\bC}} + \delta(\sum_{ij}|\gamma_{ij}|^p)^{2/p}.
% \end{equation}
% Problem (\ref{eqn:squaredPnorm}) can be equivalently reformulated in the minimax framework (\ref{eqn:minimaxGeneralAdditiveNoise}) by setting $\Omega(\bN)=\frac{1}{\delta}(\sum_{ij}|\bN_{ij}|^q)^{2/q}$, where $q$ is the dual-norm of $p$, i.e., $\frac{1}{p} + \frac{1}{q} = 1$. 

% \textbf{Schatten $p$-norm regularization}: A nuclear-norm (Schatten $1$-norm) regularization over the coupling $\gamma$ promotes a low-rank representation of the transport plan $\gamma$. Recently,   a low-rank factored transport plan $\gamma$ has been proposed in \citep{forrow19a}. The general Schatten $p$-norm ($p\geq 1$) regularized on OT formulation may be written as
% \begin{equation}\label{eqn:squaredSchattenPnorm}
%  \min_{\gamma\in\Pi}  \inner{\gamma,\hat{\bC}} + \delta\norm{\gamma}_{*p}^2,
% \end{equation}
% where $\norm{\cdot}_{*p}$ denotes the Schatten $p$-norm regularizer for a matrix. Problem (\ref{eqn:squaredSchattenPnorm}) may be equivalently reformulated within the minimax OT framework (\ref{eqn:minimaxGeneralAdditiveNoise}) by choosing $\Omega(\bN)=\frac{1}{\delta}\norm{\bN}_{*q}^2$, where $q$ is the dual-norm of $p$. 

% \subsection{Space of affine transformations}
% The next consider set of affine transformations of the cost matrices:
% $$\CC_{\textup{aff}}=\{\A(\hat{\bC}): \A:\R^{m\times n}\rightarrow\R^{m\times n} \textup{ is a linear operator};\Omega(\A)\leq 1 \},$$
% where $\Omega: \R^{m\times n}\rightarrow \R_{+}$ is a regularization function. The minimax OT problem that learns a robust transport plan over the set of cost functions $\CC_{\textup{aff}}$ may be written as:
% \begin{equation}\label{eqn:minimaxGeneralAffineNoise1}
%  \min_{\gamma\in\Pi}\ \max_{\bC\in\CC_{\textup{aff}}}\  \inner{\gamma,\bC}.
% \end{equation}
% The linear operator $\A$ may be parameterized in a number of ways. For instance, if we consider its form as $\A(\hat{\bC})=\hat{\bC}\bN$ and re-write the above in an equivalent Tikhonov form, we get the following optimization problem:  
% \begin{equation}\label{eqn:minimaxGeneralMultiplicativeNoise}
%  \min_{\gamma\in\Pi} \max_{\bN} \inner{\gamma,\hat{\bC}
% \bN} - \Omega(\bN).
% \end{equation} 
% Using the Fenchel duality theory, the optimization problem in (\ref{eqn:minimaxGeneralMultiplicativeNoise}) may be equivalently reformulated as 
% \begin{equation}\label{eqn:minGeneralMultiplicativeRegularizer}
%  \min_{\gamma\in\Pi}\ \Omega^{*}(\hat{\bC}^\top\gamma).
% \end{equation}
% Similarly, we may parameterize $\A(\hat{\bC})=\bC\odot\bN$, where $\odot$ denote the element-wise product (Hadamard product). Element-wise imputation of the given cost matrix may be useful in modeling scenarios where the importance of the $(i,j)$-th source-target pair is being varied. Then, problem (\ref{eqn:minimaxGeneralAffineNoise1}) may be equivalently reformulated as 
% \begin{equation}\label{eqn:minGeneralHadamardRegularizer}
%  \min_{\gamma\in\Pi}\ \Omega^{*}(\bC\odot\gamma). 
% \end{equation}


%\subsection{Robust $2$-Wasserstein distances}

%Note that one alternative to solve for the minimax OT $RKP(\Pi,\CC)$ with the above class of Mahalanobis cost functions is to get a closed-form expression of $\bM$ in terms of $\gamma$ and thus only solve for $\gamma$. However, this is computationally intensive (except probably for $p=2$) since it involves Schatten $q$-norm terms of $V_\gamma$ (note that $\bM\succeq0)$

%In the previous sections, we analyzed the setting in which noise imputes a generic cost function in the minimax OT framework. We now discuss a novel family of multiplicative noise in the popular $2$-Wasserstein distance setting (\ref{eqn:W22distance}), i.e., when the cost function is the squared Euclidean distance. 

\subsection{Element-wise $p$-norm regularization on $\bM$}\label{sec:p_norm}

We consider $\calM=\{\bM:\bM\succeq\bzero {\rm \ and \ } \norm{\bM}_{p}\leq1\}$ in (\ref{eqn:fgamma}), where $\norm{\bM}_{p}=(\sum_{ij} |\bM_{ij}|^p)^{\frac{1}{p}}$ denotes the element-wise $p$-norm on the matrix $\bM$. 


It should be noted that $\bV_\gamma$ is the second-order moment matrix of the displacements associated with a transport plan, i.e., for source and target distribution's samples $\{\bs_i\}_{i=1}^m\in\R^{d}$ and $\{\bt_j\}_{j=1}^n\in\R^d$, respectively, $\bV_\gamma=\sum_{ij} (\bs_i-\bt_j)(\bs_i-\bt_j)^\top \gamma_{ij}$. Hence, the proposed regularization on the metric $\bM$ learns appropriate weights to the individual components of $\bV_\gamma$. In contrast, the ${{\rm W}}_2^2$ distance, defined in (\ref{eqn:W22distance}), has $\bM=\bI$, which enforces the first-order displacements to be uncorrelated and have unit variance. This may be a strong assumption in real-word applications.

The family of element-wise $p$-norm regularizers includes the popular Frobenius norm at $p=2$. For $p$ in between $1$ and $2$, the entry-wise $p$-norm regularization induces a sparse structure on the metric $\bM$. A sparse Mahalanobis metric is useful for working with high dimensional features as it helps to avoid spurious correlations \citep{rosales06a,qi09a}. 
The following result provides an efficient reformulation of the robust OT problem (\ref{eqn:MahalanobisRobustOT}) with the above defined $\calM$ for a subset of the element-wise $p$-norm regularizers on $\bM$. 


%The following theorem proposes an equivalent reformulation of the robust OT problem (\ref{eqn:MahalanobisRobustOT}) when the Mahalanobis metric is regularized with element-wise $p$-norm:
\begin{Thm}\label{thm:p-norm}
Let $k\in\mathbb{N}$, $p=\frac{2k}{2k-1}$, and  $\calM=\{\bM:\bM\succeq\bzero {\rm \ and \ } \norm{\bM}_p\leq1\}$. Consider the optimization problem
\begin{equation}\label{eqn:proposed-p-norm-min}
%\begin{array}{lll}
%{\rm RKP}(\Pi,\D) & = & 
{{\rm W}}_{{\rm P}}(\mu_1,\mu_2)\coloneqq\minop_{\gamma\in\Pi(\mu_1,\mu_2)}\ \norm{\bV_\gamma}_{2k},
%\minop_{\gamma\in\Pi}\ \frac{1}{2k}\left(\frac{2k-1}{2k\lambda}\right)^{2k-1} \sum\limits_{s,t} \bV_\gamma(s,t)^{2k},
%\end{array}
\end{equation}
where $\bV_\gamma=\sum_{ij} (\bs_i-\bt_j)(\bs_i-\bt_j)^\top \gamma_{ij}$. Then, the following statements hold.
\begin{enumerate}
    %\item (\ref{eqn:proposed-p-norm-min}) is a convex optimization problem. 
    \item Problem (\ref{eqn:proposed-p-norm-min}) is a dual of  (\ref{eqn:MahalanobisRobustOT}) and the objectives of (\ref{eqn:MahalanobisRobustOT}) and  (\ref{eqn:proposed-p-norm-min}) are equal at optimality.
    \item For a given $\gamma\in\Pi(\mu_1,\mu_2)$, the optimal solution of (\ref{eqn:fgamma}) is $\bM^{*} (\gamma) =\norm{\bV_{\gamma}}_{2k}^{1-2k}(\bV_{\gamma})^{\circ(2k-1)}$, where $\bA^{\circ (k)}$ denotes the $k$-th Hadamard power of a matrix $\bA$, i.e., $\bA^{\circ (k)}(s,t)=\bA(s,t)^k$. 
    %\item Let $\gamma^{*}$ denote an optimal solution of (\ref{eqn:proposed-p-norm-min}). Then $(\gamma^{*},\bM^{*})$ is an optimal solution of (\ref{eqn:MahalanobisRobustOT}), where $\bM^{*}(s,t)=\left(\frac{2k-1}{2k\lambda}\right)^{2k-1} \bV_{\gamma}(s,t)^{2k-1}$. 
\end{enumerate}
%Then, the following problem (\ref{eqn:proposed-p-norm-min}) is a dual of ${\rm RKP}(\Pi,\calM)$ in (\ref{eqn:MahalanobisRobustOT}) and the objectives of (\ref{eqn:MahalanobisRobustOT}) and (\ref{eqn:proposed-p-norm-min}) are equal at optimality:
\end{Thm}
The proof of the above theorem involves a result derived in the context of multi-task learning in \citep{mjaw15a}. The proof details are in Section \ref{supp:sec:proof_pnorm}. It should be observed that for a given $\gamma$, the optimal $\bM^{*}(\gamma)$ is an element-wise function of the matrix $\bV_\gamma$. An implication is that the computation of $\bM^*(\gamma)$ costs $O(d^2)$. 


%The proposed robust OT formulation is as follows:
% \begin{equation}\label{eqn:proposed-minimax}
% {\rm RKP}(\Pi,\D) =  \minop_{\gamma\in\Pi} \maxop_{\bM\succeq \bzero} \inner{\bV_\gamma,\bM} - \lambda \sum\limits_{ij} |\bM_{ij}|^p.
% \end{equation}

An optimal solution $\gamma^{*}$ of (\ref{eqn:proposed-p-norm-min}) is also an optimal solution the problem:
\begin{equation}\label{eqn:proposed-p-norm-min-2}
{{\rm W}}_{{\rm P}}^{2k}=\minop_{\gamma\in\Pi(\mu_1,\mu_2)}\ \norm{\bV_\gamma}_{2k}^{2k}.
\end{equation}
From an optimization perspective the gradient expression for (\ref{eqn:proposed-p-norm-min-2}) is simpler than that of  (\ref{eqn:proposed-p-norm-min}). 





The following result establishes a general bound on the  ${{\rm W}}_{{\rm P}}$ distance in terms of the ${{\rm W}}_2^2$ ($2$-Wasserstein) distance as defined in (\ref{eqn:W22distance}).
\begin{Cor}\label{cor:p-norm}
Let $k\in\mathbb{N}$, $p=\frac{2k}{2k-1}$, $\calM=\{\bM:\bM\succeq\bzero; \norm{\bM}_p\leq1\}$, and the ${{\rm W}}_{{\rm P}}(\mu_1,\mu_2)$ distance as defined in (\ref{eqn:proposed-p-norm-min}). Then,
\begin{equation*}
    \frac{1}{d^\frac{1}{p}}{{\rm W}}_2^2(\mu_1,\mu_2)\leq {{\rm W}}_{{\rm P}}(\mu_1,\mu_2)\leq {{\rm W}}_2^2(\mu_1,\mu_2).
\end{equation*}
\end{Cor}


The proof of Corollary \ref{cor:p-norm} is in Section \ref{supp:sec:proof_bound_pnorm}.

%\textbf{Computing optimization ingredients efficiently}: 

% \subsection{The material below goes to supplementary}
% We begin by noting that that $\bV_\gamma = \bZ {\rm Diag}({\rm vec}(\gamma)) \bZ^\top$, where $\bZ$ is a $d\times mn$ matrix with $(i,j)$-th column as $(\bx_i-\by_j)$, ${\rm Diag}(\cdot)$ acts on a vector and outputs the corresponding diagonal matrix, and ${\rm vec}(\cdot)$ vectorizes a matrix in the column-major order. The Euclidean gradient of (\ref{eqn:proposed-p-norm-min-2}) is ${\rm vec}^{-1}({\rm diag}(\bZ^\top\bV_\gamma^{\circ(2k-1)}\bZ))$, where ${\rm diag}(\cdot)$ extracts the diagonal (vector) of a square matrix. \commentPJ{The Euclidean Hessian along a search direction $\dot{\gamma}$ is $({2k-1}){\rm vec}^{-1}({\rm diag}(\bZ^\top(\bV_\gamma^{\circ (2k-2)} \odot(\bZ {\rm Diag}({\rm vec}(\dot{\gamma})) \bZ^\top))\bZ))$.}

%{\color{red}\textbf{\#1 Some bounds for the above norm:} Lets consider the original cost $c(\bx,\by)=(\bx-\by)^\top\bI(\bx-\by)$ and its robust variant:  $c_\bM(\bx,\by)=(\bx-\by)^\top(d\bM)(\bx-\by)$. This implies that instead of $\bx$ we are considering data points of the form $\sqrt{d}\bM^\frac{1}{2}\bx$. From Holders inequality, we get $\bx^\top\bM\bx=\inner{\bM,\bx\bx^\top}\leq\norm{\bM}_p\norm{\bx\bx^\top}_q$, where the norms in the RHS is element-wise norms. Now $\norm{\bx\bx^\top}_2=\norm{\bx\bx^\top}_F=\sqrt{\trace(\bx\bx^\top\bx\bx^\top)}=\norm{\bx}^2$.}

%This class of cost functions has a different property than the class discussed in \citep{dhouib20a,paty19a}. The proposed family of robust Wasserstein distances performs feature selection (to be expanded further). 
%The optimization problem corresponding to ${\rm RKP}(\Pi,\D)$ may be written, in Tikhonov form, as:
%We have the following result on the proposed ${\rm RKP}(\Pi,\D)$: 

%It should be noted that the above problem is convex with respect to $\gamma$ (maxima over convex functions is convex). 
%In the following theorem, we propose an equivalent reformulation of the proposed minimax OT problem. 




% The problem (\ref{eqn:proposed-p-norm-min-2}) can be reformulated as
% \begin{equation}\label{eqn:proposed-min-compact}
% \begin{array}{lll}
% {\rm RKP}(\Pi,\D) & = & \minop_{\gamma\in\Pi}  \bone^\top\bv_\gamma^{2k},
% \end{array}
% \end{equation}
% where $\bv_\gamma$ is the vectorization of $\bV_\gamma$, i.e., $\bv_\gamma = {\rm vec}(\bV_\gamma)$. Also, $\bv_\gamma$ can be compactly written as $\bv_\gamma = \bP {\rm vec}(\gamma)$, where $\bP = [{\rm vec}((\bx_i-\by_j)(\bx_i-\by_j)^\top)]$ is a matrix of size $d^2 \times mn$ and $\rm{vec}$ is the vectorization operation. The Euclidean gradient is $2k{\rm vec}^{-1} ( \bP^\top \bv_\gamma^{2k-1} )$, where ${\rm vec}^{-1}$ is the reshaping of the vector back to the matrix dimensions. 
%The Euclidean Hessian along a search direction $\dot{\gamma}$ is $({2k-1})\left(\frac{2k-1}{2k\lambda}\right)^{2k-1} {\rm vec}^{-1}(\bP^\top ((\bv_\gamma^{2k-2})\odot(\bP {\rm vec}(\dot{\gamma}) )))$. 

% Another way to reformulate (\ref{eqn:proposed-min}) is by observing $\bV_\gamma = \bZ {\rm Diag}({\rm vec}(\gamma)) \bZ^\top$, where $\bZ$ is a $d\times mn$ matrix by stacking $(\bx_i - \by_j)$ side by side for all pairs and ${\rm Diag}$ acts on a vector and outputs a diagonal matrix. The Euclidean gradient is $\left(\frac{2k-1}{2k\lambda}\right)^{2k-1}  {\rm vec}^{-1}({\rm diag}(\bZ^\top\bV_\gamma^{2k-1}\bZ))$, where ${\rm diag}()$ extracts the diagonal of a square matrix. The Euclidean Hessian along a search direction $\dot{\gamma}$ is $({2k-1})\left(\frac{2k-1}{2k\lambda}\right)^{2k-1} {\rm vec}^{-1}({\rm diag}(\bZ^\top(\bV_\gamma^{2k-2} \odot(\bZ {\rm Diag}({\rm vec}(\dot{\gamma})) \bZ^\top))\bZ))$.


%\textbf{Special case of Frobenius norm regularization on $\bM$}: For $k=1$, we have the following simplified convex quadratic objective for the computing ${\rm W}_{{\rm E}}^{2k}$ in problem (\ref{eqn:proposed-p-norm-min-2}): $\norm{\bV_\gamma}_2^2={\rm vec}(\gamma)^\top \bA {\rm vec}(\gamma)$, where $\bA=(\bZ^\top\bZ)\odot (\bZ^\top\bZ)$ and $\odot$ denotes the Hadamard product. 
%\textbf{Special case of Frobenius norm regularization on $\bM$}: For $k=1$, we have the following simplified convex quadratic objective for the computing ${\rm W}_{{\rm E}}^{2k}$: $\norm{\bV_\gamma}_2^2={\rm vec}(\gamma)^\top \bA {\rm vec}(\gamma)$, where $\bA=(\bZ^\top\bZ)\odot (\bZ^\top\bZ)$ and $\odot$ denotes the Hadamard product. 
%In this special case of $p=2$, the proposed formulation is equivalent to the Schatten $2$-norm formulation discussed in \citep{dhouib20a}. However, \citep{dhouib20a} only discusses the general algorithm and does not explore such simplifications. 




\subsection{KL-divergence regularization on $\bM$}\label{sec:KL}


We next consider the generalized KL-divergence regularization on the metric $\bM$, i.e., $\calM=\{\bM:\bM\succeq\bzero;{{\rm D}_{\rm KL}}(\bM,\bM_0)\leq 1\}$, where ${{\rm D}_{\rm KL}}(\bM,\bM_0)=\sum_{s,t} \bM_{st}(\ln{\left(\bM_{st}/{\bM_0}_{st}\right)})-(\bM_{st} - {\bM_{0}}_{st})$ denotes the Bregman distance, with negative entropy as the distance-generating function, between the matrices $\bM$ and $\bM_0\succeq\bzero$. Here, $\bM_0$ is a given symmetric positive semi-definite matrix, which may be useful in introducing a prior domain knowledge (e.g., a block diagonal matrix $\bM_0$ ensures grouping of features). 
%A default choice of $\bM_0$ is  $\bM_0=\bone\bone^\top$, where all the features are equally correlated (similar) with each other. 
The function $f(\gamma)$ in (\ref{eqn:fgamma}) with the above defined $\calM$ may be expressed in the Tikhonov form as
%This regularization ensures that the entries of $\bM$ are positive. Hence, the domain of $\bM$ is the set of positive-definite matrices with positive entries. 
\begin{equation}\label{eqn:proposed-minimax-kl-divergence}
f(\gamma) = \maxop_{\bM\succeq \bzero}\  \inner{\bV_\gamma,\bM}-\lambda_{\bM} {{\rm D}_{\rm KL}}(\bM,\bM_0),
\end{equation}
% \begin{equation}\label{eqn:proposed-minimax-kl-divergence}
% {{\rm W}}_{{\rm KL}}(\mu_1,\mu_2) = \minop_{\gamma\in\Pi} \maxop_{\bM\succeq \bzero}\  \inner{\bV_\gamma,\bM}- \lambda_{\bM} {{\rm D}_{\rm KL}}(\bM,\bM_0),
% \end{equation}
where $\lambda_{\bM}>0$ is a regularization parameter. The following result provides an efficient reformulation of the KL-divergence regularized robust OT problem. 
\begin{Thm}\label{thm:kl-regularization}
%Consider the KL-divergence regularized robust OT problem (\ref{eqn:MahalanobisRobustOT}), where $f(\gamma)$ is as defined in (\ref{eqn:proposed-minimax-kl-divergence}). 
The following problem is an equivalent dual of the convex problem (\ref{eqn:MahalanobisRobustOT}) where $f(\gamma)$ is as defined in (\ref{eqn:proposed-minimax-kl-divergence}):
\begin{equation}\label{eqn:proposed-min-kl-divergence}
\begin{array}{lll}
%W_{KL}(\mu_1,\mu_2) = \minop_{\gamma\in\Pi} \lambda \sum\limits_{s,t} \bM_0(s,t)(e^{\bV_\gamma(s,t)/\lambda}-1).
{{\rm W}}_{{\rm KL}}(\mu_1,\mu_2) =   \minop_{\gamma\in\Pi(\mu_1,\mu_2)} \lambda_{\bM} \bone^\top( \bM_0\odot e^{\circ (\bV_\gamma/\lambda_{\bM})} - \bM_0)\bone,
\end{array}
\end{equation}
where $e^{\circ\bA}$ denotes the Hadamard exponential (element-wise exponential) of a matrix $\bA$. For a given $\gamma\in\Pi(\mu_1,\mu_2)$, the optimal solution of  (\ref{eqn:proposed-minimax-kl-divergence}) is  $\bM^{*}(\gamma)=\bM_0\odot e^{\circ (\bV_{\gamma}/\lambda_{\bM})}$. 
\end{Thm}
% It should be noted that the optimal solution $\gamma^{*}$ of (\ref{eqn:proposed-min-kl-divergence}) with $\bM_0=\bone\bone^\top$ is also the optimal solution of the problem:
% \begin{equation}\label{eqn:proposed-min-log-sum-exp}
% %\begin{array}{lll}
% {{\rm W}}_{{\rm S}}(\mu_1,\mu_2)=\minop_{\gamma\in\Pi(\mu_1,\mu_2)} \lambda \log{\left(\sum\limits_{s,t} e^{\bV_\gamma(s,t)/\lambda}\right)}.
% %\end{array}
% \end{equation}
% The objective in (\ref{eqn:proposed-min-log-sum-exp}) is a log-sum-exp function on the entries of the matrix $\bV_\gamma$, which is a smooth approximation of the maximum function. Thus, the optimal $\gamma^{*}$ in (\ref{eqn:proposed-min-log-sum-exp}) minimizes (a smooth approximation of) the maximum over the  entries of $\bV_\gamma$. Interestingly, problem (\ref{eqn:proposed-min-log-sum-exp}) is equivalent to the robust OT problem (\ref{eqn:MahalanobisRobustOT}) with $f(\gamma)$ defined as 
% \begin{equation}\label{eqn:proposed-minimax-log-sum-exp}
% f(\gamma) =  \maxop_{\bM\in\calM} \inner{\bV_\gamma,\bM} - \lambda {{\rm D}_{\rm KL}}(\bM,\bone\bone^\top),
% \end{equation}
% where $\calM=\{\bM:\bM\succeq \bzero;\bM>\bzero;\bone^\top\bM\bone=1\}$. We observe that problem (\ref{eqn:proposed-minimax-log-sum-exp}) learns a positive semi-definite Mahalanobis metric whose entries lies on a $(mn-1)$-dimensional simplex \commentPJ{(without a boundary)}. 
We next analyze the doubly-stochastic structure on $\bM$. 


\subsection{Doubly-stochastic regularization on $\bM$}\label{sec:doubly_stochastic}


We consider the robust OT problem (\ref{eqn:MahalanobisRobustOT}) in which the metric $\bM$ is also doubly-stochastic, i.e.,
\begin{equation}\label{eqn:proposed-minimax-doubly-stochastic}
%{{\rm W}}_{{\rm DS}}(\mu_1,\mu_2) = \minop_{\gamma\in\Pi} \maxop_{\bM\in\calM}\ \inner{\bV_\gamma,\bM},
f(\gamma) = \maxop_{\bM\in\calM}\ \inner{\bV_\gamma,\bM},
\end{equation}
where $\calM=\{\bM:\bM\succeq\bzero ,\bM \geq\bzero, {\rm \ and \ }\bM\bone=\bone\}$. 
Learning of doubly-stochastic Mahalanobis metric is of independent interest in  applications such as graph clustering and community detection \citep{zass06a,arora11a,wang16a,douik18a,douik2019manifold}. %In our case, the doubly-stochastic constraint on $\bM$ allows to capture natural associations among various components of the second-order moment matrix $\bV_\gamma$. 


In general, optimization over the set of positive semi-definite stochastic matrices is non trivial and computationally challenging. By exploiting the problem structure, however, we show that (\ref{eqn:proposed-minimax-doubly-stochastic}) can be solved efficiently by adding a small KL-divergence regularization. To this end, we propose to solve for
\begin{equation}\label{eqn:proposed-max-doubly-stochastic-regularized}
\Tilde{f}(\gamma) =
\maxop_{\bM\in\calM}\ \inner{\bV_\gamma,\bM} - \lambda_{\bM}{{\rm D}_{\rm KL}}(\bM,\bM_0),
\end{equation}
where $\lambda_{\bM}>0$ is a small regularization parameter and $\bM_0$ is a symmetric positive semi-definite prior which is also element-wise positive. Our next result discusses the solution of (\ref{eqn:proposed-max-doubly-stochastic-regularized}). 
\begin{Thm}\label{thm:doubly-stochastic-regularization}
For a given $\gamma\in\Pi(\mu_1,\mu_2)$, the optimal solution of (\ref{eqn:proposed-max-doubly-stochastic-regularized}) has the form $\bM^{*}(\gamma)=\bD\left( \bM_0 \odot e^{\circ(\bV_\gamma/\lambda_{\bM})}\right)\bD$, where $\bD$ is a diagonal matrix with positive entries. 
\end{Thm}
The matrix $\bD$ in Theorem~\ref{thm:doubly-stochastic-regularization} is efficiently computed using the Sinkhorn algorithm \citep{cuturi13a}. 










\section{Robust optimal transport with low-dimensional metric $\bM$} \label{sec:low_dimensional_metric_decomposition}




Section \ref{sec:formulations} discusses several regularizations on the Mahalanobis metric $\bM$ that lead to efficient computation of $\bM^{*}(\gamma)$, i.e., the solution to  (\ref{eqn:fgamma}). For a given $\bV_\gamma$, computation of $\bM^{*}(\gamma)$, for regularizations considered in Section \ref{sec:formulations}, requires $O(d^2)$, which though linear in the size of $\bM$, may be prohibitive for  high-dimensional data. 

In this section, we discuss a particular dimensionality reduction technique that addresses the computational issue. To this end, we propose a novel decomposition of the Mahalanobis metric $\bM$ as 
%We propose to \changeBM{decompose} the Mahalanobis metric $\bM$ as follows:
\begin{equation}\label{eqn:factorizeMahalanobis}
    \bM=\bB\otimes\bI_{d_1},
\end{equation}
where $\otimes$ denotes the Kronecker product, $\bI_{d_1}$ denotes the identity matrix of size $d_1 \times d_1$, and  $\bB\succeq\bzero$ is a $r\times r$ symmetric positive semi-definite matrix such that $d=d_1r$, where $r \ll d$. The decomposition (\ref{eqn:factorizeMahalanobis}) induces the following reformulation of the objective in (\ref{eqn:fgamma}) as
\begin{equation}\label{eqn:reshaping}
\begin{array}{lll}
    \inner{\bV_\gamma,\bB\otimes\bI_{d_1}}
    &=& \inner{\sum_{ij}\gamma_{ij}(\bs_i-\bt_j)(\bs_i-\bt_j)^\top,\bB\otimes\bI_{d_1}}\\
    &=& \inner{\sum_{ij}\gamma_{ij}(\bS_i-\bT_j)^\top(\bS_i-\bT_j),\bB}\\
    &=& \inner{\bU_\gamma, \bB},
\end{array}
\end{equation}
where $\bS_i$ and $\bT_j$ are $d_1\times r$ matrices obtained by reshaping the vectors $\bs_i$ and $\bt_j$, respectively. 


We observe that the proposed decomposition of the Mahalanobis metric (\ref{eqn:factorizeMahalanobis}) divides the $d$ features into $r$ groups, each with $d_1$ input features. Based on (\ref{eqn:reshaping}), the symmetric positive semi-definite matrix $\bB$ may be viewed as a Mahalanobis metric over the feature groups. In addition, it can be shown that any proposed regularization on the metric $\bM$ (in Section~\ref{sec:formulations}) transforms into an equivalent regularization on the ``group'' metric $\bB$. 

The function $f(\gamma)$, in the robust optimal transport problem (\ref{eqn:MahalanobisRobustOT}), is equivalently re-written as
\begin{equation}\label{eqn:factorizeMahalanobisRobustOT}
    f(\gamma) = \max_{\bB\in\calB}\ \inner{\bU_\gamma,\bB},
\end{equation}
where $\calB=\{\bB:\bB\succeq\bzero {\rm \ and \ } \Omega(\bB) \leq 1\}$. For the regularizers discussed in Section \ref{sec:formulations}, the computation of the solution $\bB^*(\gamma)$ of (\ref{eqn:factorizeMahalanobisRobustOT}) costs $O(r^2)$. 









\section{The Frank-Wolfe algorithm for (\ref{eqn:MahalanobisRobustOT})}\label{sec:algorithms}

The formulations proposed in Section \ref{sec:formulations} are expressed as minimization of a non-linear convex function $f: \Pi \rightarrow \mathbb{R} : \gamma \mapsto f(\gamma)$ over $\Pi(\mu_1, \mu_2)$. Here, the objective function $f$ encapsulates the Mahalanobis metric $\bM$ and is more generically written as $f(\gamma) \coloneqq  \max_{\bM \in \mathcal{M}} \langle \bV_{\gamma},  \bM\rangle$. 


A popular way to solve a convex constrained optimization problem (\ref{eqn:MahalanobisRobustOT}) is with the Frank-Wolfe (FW) algorithm, which is also known as the conditional gradient algorithm. It requires solving a constrained linear minimization sub-problem (LMO) at every iteration. For many convex constraints, the LMOs are often easy to solve, thereby making the FW algorithm an appealing choice in practice \citep{jaggi2013revisiting}.

The proposed algorithm  for (\ref{eqn:MahalanobisRobustOT}) is shown in Algorithm \ref{alg:FW}. The LMO step boils down to solving the optimal transport problem (\ref{eqn:optimal-transport}), where the cost matrix is replaced by $\nabla_{\gamma} f$. When regularized with an entropy regularization term, the LMO step admits a computationally efficient solution using the Sinkhorn algorithm \citep{cuturi13a}.



\begin{algorithm}[tb]
   \caption{Proposed FW algorithm for (\ref{eqn:MahalanobisRobustOT})}
   \label{alg:FW}
   {%\footnotesize
    %\begin{tabular}{ l | l }
  {\bfseries Input:} Source distribution's samples $\{\bs_i\}_{i=1}^m\in\R^{d}$ and target distribution's samples $\{\bt_j\}_{j=1}^n\in\R^{d}$. Initialize $\gamma_0 \in \Pi(\mu_1, \mu_2)$. 
   
  {\bfseries for} $t = 0\ldots T$ {\bfseries do} 
  
  \qquad Compute $\nabla f_{\gamma}(\gamma_t)$ using Lemma \ref{lemma:gradient_and_directional_derivative}.
  
  
  \qquad LMO step: Compute $\hat{\gamma}_t\coloneqq \argmin_{\beta \in \Pi(\mu_1,\mu_2)} \langle \beta, \nabla f_{\gamma}(\gamma_t)\rangle$.
  
  
  \qquad Update $\gamma_{t+1} = (1-\theta)\gamma_t + \theta \hat{\gamma}_t$ for $\theta = \frac{2}{t+2}$.
 
  {\bfseries end for}

{\bfseries Output:} $\gamma^*$ and $\bM^* = \bM^*(\gamma^*)$.
%    \end{tabular}
    }
\end{algorithm}



 We now develop the expression of $\nabla_{\gamma} f$ and discuss its computational cost. We begin by noting that $\bV_\gamma = \bZ {\rm Diag}({\rm vec}(\gamma)) \bZ^\top$, where $\bZ$ is a $d\times mn$ matrix with $(i,j)$-th column as $(\bs_i-\bt_j)$, ${\rm Diag}(\cdot)$ acts on a vector and outputs the corresponding diagonal matrix, and ${\rm vec}(\cdot)$ vectorizes a matrix in the column-major order. 

\begin{Lem}\label{lemma:gradient_and_directional_derivative}
Let $\bM^*(\gamma_t)$ be the solution to the problem $\maxop_{\bM \in \mathcal{M}} \langle \bV_{\gamma_t},  \bM\rangle$ for a given $\gamma_t \in \Pi(\mu_1,\mu_2)$. Then, the gradient $\nabla_{\gamma} f (\gamma_t)$ of $f$ in (\ref{eqn:MahalanobisRobustOT}) with respect to $\gamma$ has the expression 
\begin{equation*}
    \nabla_{\gamma} f(\gamma_t) = {\rm vec}^{-1}({\rm diag}(\bZ^\top \bM^*(\gamma_t)\bZ)), 
\end{equation*}
where ${\rm diag}(\cdot)$ extracts the diagonal (vector) of a square matrix and ${\rm vec}^{-1}$ reshapes a vector into a matrix. 

\end{Lem}

The proof of Lemma \ref{lemma:gradient_and_directional_derivative} is in Section \ref{supp:sec:proof_gradient}. Lemma \ref{lemma:gradient_and_directional_derivative} shows that the gradient $\nabla_{\gamma} f $ can be written by using $\bM^*(\gamma)$. For the formulations presented in Section \ref{sec:formulations}, the expressions for $\bM^*(\gamma)$ can be computed efficiently. Overall, the computation of $\nabla_{\gamma} f$ costs $O(mnd^2)$.

For the cost function (\ref{eqn:factorizeMahalanobisRobustOT}) obtained with the $r$-dimensional decomposition of $\bM$, Lemma \ref{lemma:gradient_and_directional_derivative} can be appropriately modified. In this case, the cost of computation of $\nabla_{\gamma} f $ is $O(mnr^2)$.







% \subsection{Manifold approach}\label{sec:manifold}


% Another approach is by exploiting the fact that $\Pi(\mu_1,\mu_2)$ has a smooth manifold structure for $\gamma > 0$, i.e., strict positivity of the entries of $\gamma$ \citep{douik2019manifold,shi19a}. In particular, we use the Riemannian optimization framework that 
% conceptually translates a constrained optimization problem of the form (\ref{eqn:MahalanobisRobustOT}) into an {\it unconstrained} optimization problem over the manifold $\Pi(\mu_1,\mu_2)$. It allows to build first- and second-order algorithms over $\Pi(\mu_1,\mu_2)$ systematically, thereby allowing to use conjugate gradients and trust-regions algorithms \citep{absil2009optimization,boumal2020intromanifolds}.


% $\Pi(\mu_1,\mu_2)$ is endowed with the {\it Fisher} information metric, as the Riemannian metric, defined as \citep{douik2019manifold,shi19a,sun2015heterogeneous}
% \begin{equation}\label{eqn:Riemannian_metric}
%     \begin{array}{ll}
%          g_{\gamma}(\eta_{\gamma}, \xi_{\gamma}) \coloneqq 
%          \trace((\eta_{\gamma} \odot \xi_{\gamma}) \oslash \gamma),
%     \end{array}
% \end{equation}
% where $\eta_{\gamma}$ are $ \xi_{\gamma}$ tangent vectors belonging to the tangent space $T_{\gamma} \Pi(\mu_1,\mu_2) \coloneqq \{ \zeta_{\gamma} \in \mathbb{R}^{m\times n} : \zeta_{\gamma} \bone = 1/m, \zeta_{\gamma}^\top \bone =  1/n \}$ at $\gamma$. Here, $\odot$ and $\oslash$ are element-wise matrix multiplication and division, respectively. The Riemannian metric (\ref{eqn:Riemannian_metric}) scales the boundary of $\Pi(\mu_1,\mu_2)$ to ``infinity'', i.e., as $\gamma_{ij}$ tends to zero, the inner product tends to infinity, thereby endowing $\Pi(\mu_1,\mu_2)$ with a smooth {\it differentiable} structure. \changeBM{This is in contrast to the FW approach in Section \ref{sec:FW} where an entropy term has to be added explicitly in the LMO step.}


% %It is interesting to note that the Fisher metric (\ref{eqn:Riemannian_metric}) is same as the popular Bures-Wasserstein metric (defined for the manifold of symmetric positive definite matrices) when restricted to positive scalars \citep{bhatia2019bures,malago2018wasserstein}.  


% The Riemannian conjugate (CG) gradient and trust-regions (TR) algorithms require the notions of Riemannian {\it gradient} (the steepest descent direction on the manifold) and {\it Hessian} (the covariant derivative of the Riemannian gradient), which admit simple formulas in terms of $\nabla f$ and its directional derivative ${\rm D} \nabla f(\gamma)[\dot{\gamma}]$, respectively \citep{douik2019manifold,sun2015heterogeneous}. Moving along the manifold is captured with the notion of a {\it retraction} operator (ensures that we always stay on the manifold) which has a well-defined expression using the Sinkhorn-Knopp algorithm \citep{douik2019manifold}.



% %Conceptually, the Riemannian optimization framework translates a constrained optimization problem of the form (\ref{eqn:manifold_optimization}) into {\it unconstrained} optimization over the manifold $\Pi$. Accordingly, standard notions of optimization like gradient (the descent direction of a function on the manifold), Hessian (the second-order derivatives of a function), updates on the manifold (moving along the shortest path on the manifold), and transport of (tangent) vectors are generalized to the manifold space. Those expressions have easy-to-implement numerical formulas for the manifold $\Pi$ given any smooth function $f$ \citep{douik2019manifold}.






 



% \section{Related work}
% For a given $\gamma$, the worst case Mahalanobis metric parameterized cost function with the Schatten $p$-norm regularization is given by \citep[Proposition 1]{dhouib20a}:
% \begin{equation}\label{eqn:schatten-norm}
%     \bM^{*}(\gamma) = \argmax\limits_{\bM\succeq\bzero, \norm{\bM}_{*p}\leq1} \inner{\bV_\gamma,\bM}=\left(\frac{\bV_\gamma}{\norm{\bV_\gamma}_{*q}}\right)^{\frac{q}{p}},
% \end{equation}
% where $\norm{\cdot}_{*p}$ denotes the Schatten $p$-norm and $q$-norm is the dual of $p$-norm. Computing $\bM^{*}(\gamma)$ in (\ref{eqn:schatten-norm}) is relatively simple for $p=\{1,2,\infty\}$ but requires eigenvalue decomposition of the matrix $\bV_\gamma$ for other values of $p$. This is due to the positive semi-definite (PSD) constraint over the matrix $\bM$. In this regard, \citep{dhouib20a} has remarked that \textit{``PSD constraints increase considerably the computational burden of any optimization problem, yet they are necessary for the obtained cost function to be a true metric.''}

% \citep{dhouib20a} also analyze the minimax OT problem where the worst case cost function belongs to a convex hull of a finite number of cost functions. Hence, if $\{c_1,\ldots,c_K\}$ is a given set of cost functions, then the search space of the cost functions is $c=\sum_{i=1}^K \alpha_i c_i$, where $\alpha$ lies on a $K-1$ dimensional simplex polytope ($\sum_i \alpha_i=1, \alpha_i\geq 0\ \forall i$).  


\section{Learning with robust optimal transport loss}\label{sec:ROTloss}

Optimal transport based distances provide a natural metric on the output space, and hence, can be used to in learning problems. Specifically, \citet{frogner15a} discuss the multi-label classification problem set up where they employ the Wasserstein distance as the loss function. 

In this section, we discuss the use of the robust OT distance as a loss function in learning problems. We begin by explaining the learning problem setup with ${\rm W}_{\rm ROT}$ as a loss function. We then discuss the qualitative nature of the proposed robust OT distance-based loss functions and present an efficient way to compute the gradient of the robust OT distance loss. Later in Section~\ref{sec:experiments}, we empirically demonstrate the effectiveness of using ${\rm W}_{\rm ROT}$ as loss function in supervised multi-label/multi-class classification problems. 

\subsection{Problem setup}
Consider the standard multi-label (or multi-class) problem over $L$ labels (classes) and given supervised training instances $\{\bx_j,\by_j\}_{j=1}^N$. Here, $\bx_j\in\R^M$ and $\by_j\in\{0,1\}^L$. The prediction function of $p$-th label is given by the {\it softmax} function
\begin{equation}\label{eqn:softmax}
    h_p(\bx;\bW)=\frac{e^{\inner{\bw_p,\bx}}}{\sum_{l=1}^L e^{\inner{\bw_l,\bx}}},
\end{equation}
where $\bW=[\bw_1,\ldots,\bw_L]$ is the model parameter of the multi-label problem. The prediction function $h(\bx;\bW)$ can be learned via the empirical risk minimization framework. 


\citet{frogner15a} use the Wasserstein distance as the loss function for multi-label classification problem as follows. For an input $\bx_j$, the prediction function $h(\bx_j;\bW)$ in Equation~(\ref{eqn:softmax}) may be viewed as a discrete probability distribution. Similarly, a $0-1$ binary ground-truth label vector $\by_j$ may be transformed into a discrete probability distribution by appropriate normalization: $\hat{\by}_j=\by_j/\by_j^\top \bone$ \citep{frogner15a}. Given a suitable ground cost metric between the labels, the Wasserstein distance is employed to measure the distance between the prediction $h(\bx_j;\bW)$ and the ground-truth $\hat{\by}_j$. If the labels correspond to real-word entities, then a possible ground cost metric may be obtained from the word embedding vectors corresponding to the labels \citep{mikolov13a,bojanowski16a}. 

\begin{figure}[t]
\center
\includegraphics[width=.8\textwidth]{figs/RboTvsM22_Siamese+cat_Elephant_kl_1e-2.pdf}
\caption{Contour plots of various OT distance based loss functions. The labels are \{`Siamese$\_$cat', `Elephant', `Persian$\_$cat'\}, with `Persian$\_$cat' as the true label. The plots show the relative loss incurred by various possible predictions of the form $\bh=[x,y,1-x-y]^\top$, where $0\leq x,y\leq1$ and $x+y\leq 1$. We observe linear contours for the ${\rm W}_2^2$ loss function while non-linear contours for the proposed robust OT loss functions: ${\rm W}_{\rm P}$ with $k=1$, ${\rm W}_{\rm KL}$, and ${\rm W}_{\rm DS}$. The robust OT loss functions relatively penalize `Siamese$\_$cat' lesser than `Elephant', i.e., more lighter color in the feasible $x>y$ regions in plots (b), (c), and (d) than in plot (a). }\label{fig:cce}
\end{figure}


\begin{figure}[t]
\center
\includegraphics[width=.8\textwidth]{figs/RboTvsM22_Blue+whale_Elephant_kl_1e-2.pdf}
\caption{Contour plots of various OT distance based loss functions. The labels are \{`Blue$\_$whale', `Elephant', `Persian$\_$cat'\}, with `Persian$\_$cat' being the true label. All three classes are quite dissimilar from each other. Hence, all OT based loss functions relatively penalize both the incorrect classes similarly.}\label{fig:cwe}
\end{figure}



\begin{figure}[t]
\center
\includegraphics[width=.8\textwidth]{figs/RboTvsM22_Blue_whale_Dolphin_kl_1e-2.pdf}
\caption{Contour plots of various OT distance based loss functions. The labels are \{`Blue$\_$whale', `Dolphin', `Humpback$\_$whale'\}, with `Humpback$\_$whale' as the true label. All three classes share similar characteristics but `Blue$\_$whale is more similar to `Humpback$\_$whale'.}\label{fig:llt}
\end{figure}

\subsection{Multi-label learning with the ${\rm W}_{\rm ROT}$ loss}
We propose to employ the robust OT distance-based loss in multi-label/multi-class problems. To this end, we solve the empirical risk minimization problem, i.e.,
\begin{equation}\label{eqn:multi-label}
    \minop_{\bW\in\R^{M\times L}}\ \frac{1}{N} \sum_{j=1}^N{\rm W}_{\rm ROT}(h(\bx_j;\bW),\hat{\by}_j),
\end{equation}
where ${\rm W}_{\rm ROT}$ is the robust OT distance-based function  (\ref{eqn:MahalanobisRobustOT}). Here, ${\rm W}_{\rm ROT}$ may be set to any of the discussed robust OT distance functions such as ${\rm W}_{\rm P}$ (\ref{eqn:proposed-p-norm-min}), ${\rm W}_{\rm KL}$ (\ref{eqn:proposed-min-kl-divergence}), and ${\rm W}_{\rm DS}$ (\ref{eqn:proposed-max-doubly-stochastic-regularized}). As discussed, \citet{frogner15a} employ ${\rm W}_p^p(h(\bx;\bW),\hat{\by})$ as the loss function in (\ref{eqn:multi-label}).

We analyze the nature of the ${\rm W}_2^2$-based loss function and the proposed ${\rm W}_{\rm ROT}$-based loss functions by viewing their contours plots for the three-class setting. We consider the labels as \{\textit{A},\textit{B},\textit{C}\}. We consider label \textit{C} as true label, i.e., $\hat{\by}=[0,0,1]^\top$, where the first dimension corresponds to label \textit{A} and consider predictions of the form $\bh=[a,b,1-a-b]$. 
Since $h$ is obtained from the softmax function (\ref{eqn:softmax}), we have $(a,b) \in \{(x,y):0\leq x,y\leq 1 {\rm \ and \ }x+y\leq 1\}$. The ground cost function is computed using the fastText word embeddings corresponding to the labels \citep{bojanowski16a}.

We plot the contour maps of the ${\rm W}_2^2(\bh,\hat{\by})$ loss function and the proposed ${\rm W}_{\rm P}(\bh,\hat{\by})$, ${\rm W}_{\rm KL}(\bh,\hat{\by})$, and ${\rm W}_{\rm DS}(\bh,\hat{\by})$ loss functions, as $(a,b)$ varies along the two-dimensional $X-Y$ plane. All the plots are made to same scale by normalizing the highest value of the loss to $1$.

In Figure~\ref{fig:cce}, we consider the labels as \{\textit{A},\textit{B},\textit{C}\}=\{`Siamese$\_$cat', `Elephant', `Persian$\_$cat'\}. The first and the third classes in this setting are similar, and the OT distance based loss functions should exploit this relationship via the ground cost function. With `Persian$\_$cat' as the true class, we observe that the all four losses in Figure~\ref{fig:cce} penalize `Elephant' more than `Siamese$\_$cat'. However, the contours of ${\rm W}_2^2$ loss in  Figure~\ref{fig:cce}(a) are linear, while those of the proposed ${\rm W}_{\rm P}$ with $k=1$ Figure~\ref{fig:cce}(b) are elliptical. On the other hand, the proposed ${\rm W}_{\rm KL}$ and ${\rm W}_{\rm DS}$ exhibit varying degree of non-linear contours (modeled by $\lambda_{\bM}$ parameter). Overall, the proposed robust OT distance based loss functions penalize 'Siamese$\_$cat' relatively lesser than the ${\rm W}_2^2$  loss.

In Figure~\ref{fig:cwe}, we consider the labels as \{\textit{A},\textit{B},\textit{C}\}=\{'Blue$\_$cat', 'Elephant', 'Persian$\_$cat'\}. The two classes `Blue$\_$cat' and `Elephant' are quite dissimilar to the true class `Persian$\_$cat'. We observe that while the ${\rm W}_2^2$ loss exhibits similar linear contours as previously (but with a different slope),  non-linearity in the proposed robust OT based losses allow them more freedom to adapt. 
We provide contour maps for another interesting setting, where all the three classes are similar, but one class is more closer to the true class. In Figure~\ref{fig:llt}, we consider the labels as \{\textit{A},\textit{B},\textit{C}\}=\{'Blue$\_$whale', 'Dolphin', 'Humpback$\_$whale'\}.





\begin{table*}[t]
  \caption{Generalization performance of various optimal transport based loss functions on the supervised multi-class/multi-label problems.}\label{table:results}
  \begin{center}
    \begin{tabular}{lccccc}
      \toprule
      \multirow{2}{*}{Method} & \multirow{2}{*}{$r$} & Animals & MNIST & \multicolumn{2}{c}{Flickr} \\ 
      & & (AUC) & (AUC) & (AUC) & (mAP) \\
      \midrule
      \multirow{1}{*}{${\rm W}_2^2$} loss \citep{frogner15a} & $-$ & $0.794$ & $0.848$ & $0.649$ & $0.0209$\\
      \midrule
      \multirow{3}{*}{${\rm W_{P}}$ loss with $k=1$  (Eq.~\ref{eqn:proposed-p-norm-min})} & $5$ & $0.801$ & $\mathbf{0.959}$ & $0.706$ & $0.0481$\\
      & $10$ & $0.907$ & $0.940$ & $0.745$  & $0.0625$\\
      & $20$ & $\mathbf{0.908}$ & $0.922$ & $\mathbf{0.768}$  & $\mathbf{0.0717}$\\
      \midrule
      \multirow{3}{*}{${\rm W_{P}}$ loss with $k=2$ (Eq.~\ref{eqn:proposed-p-norm-min})} & $5$ & $0.890$ & $0.804$ & $0.760$  & $0.0625$\\
      & $10$ & $0.878$ & $0.702$ & $0.742$  & $0.0468$\\
      & $20$ & $0.874$ & $0.603$ & $0.737$  & $0.0441$\\
      \midrule
      \multirow{3}{*}{${\rm W_{KL}}$ loss  (Eq.~\ref{eqn:proposed-min-kl-divergence})} & $5$ & $0.794$ & $0.867$ & $0.648$  & $0.0207$\\
      & $10$ & $0.749$ & $0.870$ & $0.649$  & $0.0205$\\
      & $20$ & $0.794$ & $0.779$ & $0.649$  & $0.0205$\\
      \midrule
      \multirow{3}{*}{${\rm W_{DS}}$ loss  (Eq.~\ref{eqn:proposed-max-doubly-stochastic-regularized})} & $5$ & $\mathbf{0.908}$ & $0.927$ & $0.724$  & $0.0530$\\
      & $10$ & $0.878$ & $0.873$ & $0.668$  & $0.0325$\\
      & $20$ & $0.845$ & $0.813$ & $0.628$  & $0.0219$\\
      \bottomrule
    \end{tabular}
  \end{center}
\end{table*}


\subsection{Optimizing the ${\rm W}_{\rm ROT}$ loss}

We solve Problem (\ref{eqn:multi-label}) using the standard stochastic gradient descent (SGD) algorithm. In each iteration of the SGD algorithm, we pick a training instance $j = \{1, \ldots, N \}$ and update the parameter $\bW$ along the negative of the gradient of the loss term ${\rm W}_{\rm ROT}(h(\bx_j;\bW),\hat{\by}_j))$ with respect to the model parameter $\bW$. 

We obtain it using the chain rule by computing $\nabla_\bW h(\bx_j;\bW)$ and $\nabla_{h(\bx;\bW)} {\rm W}_{\rm ROT}(h(\bx_j;\bW),\hat{\by}_j)$. While the expression for $\nabla_\bW h(\bx_j;\bW)$ is well studied, computing $\nabla_{h(\bx;\bW)} {\rm W}_{\rm ROT}(h(\bx_j;\bW),\hat{\by}_j)$ is non trivial as the loss ${\rm W}_{\rm ROT}(h(\bx_j;\bW),\hat{\by}_j)$ involves a min-max optimization problem  (\ref{eqn:MahalanobisRobustOT}). To this end, we consider a regularized version of ${\rm W}_{\rm ROT}$ by adding a negative entropy regularization term to (\ref{eqn:fgamma}). Equivalently, we consider the formulation for computing the robust OT distance between $h(\bx_j;
\bW)$ and $\hat{\by}_j$ as
\begin{equation}\label{eqn:rotminmax}
\begin{array}{ll}
  {\rm W}_{\rm ROT}(h(\bx_j;\bW),\hat{\by}_j) =  
   \minop_{\gamma \in \Pi(h(\bx_j;\bW),\hat{\by}_j)} \maxop_{\bM \in \calM} \inner{\bV_\gamma,\bM} + 
   \lambda_{\gamma} \sum_{pq} \gamma_{pq} {\rm ln}(\gamma_{pq}),
  \end{array}
\end{equation}
where $\lambda_{\gamma} >0$ and $\bV_{\gamma} = \sum_{pq} (\bl_p - \bl_q)(\bl_p - \bl_q)^\top \gamma_{pq}$ is of size $L \times L$. Here, $\bl_p$ is the ground embedding of $p$-th label. 








The following lemma provides an expression for the gradient of ${\rm W}_{\rm ROT}(h(\bx_j;\bW),\hat{\by}_j)$ with respect to $h(\bx; \bW)$.

\begin{Lem}\label{lemma:gradient_rot}
Let $(\gamma^{*}, \bM^*(\gamma^*))$ denote the optimal solution of the robust OT problem (\ref{eqn:rotminmax}). Then, 
\begin{equation}\label{eqn:gradient_rot}
\begin{array}{lll}
\nabla_{h(\bx;\bW)} {\rm W}_{\rm ROT}(h(\bx_j;\bW),\hat{\by}_j) =  \frac{1}{L}\bA \bone - \frac{\bone ^\top \bA \bone}{L^2} \bone,
\end{array}
\end{equation}
where $\bone $ is the column vector of ones of size $L$ and $\bA = \bC^*+ \lambda_{\gamma } ({\rm ln}(\gamma ^*) + \bone \bone^\top)$. Here, $\bC^*_{pq} = (\bl_p - \bl_q)^\top \bM^*(\gamma^*) (\bl_p - \bl_q)$.
\end{Lem}

The proof of Lemma \ref{lemma:gradient_rot} is in Section \ref{supp:sec:proof_gradient_rot}. 

For the multi-label setting, computation of the gradient $\nabla_{h(\bx;\bW)} {\rm W}_{\rm ROT}(h(\bx_j;\bW),\hat{\by}_j)$, shown in (\ref{eqn:gradient_rot}), in Lemma \ref{lemma:gradient_rot} costs $O(l_j Ld^2)$, where $l_j$ is the number of ground-truth labels for the $j$-th training instance. Using the decomposition (\ref{eqn:factorizeMahalanobis}), the cost reduces to $O(l_jLr^2)$. In many cases, $l_j$ is much smaller than $L$. 

For the multi-class setting, computation of the gradient $\nabla_{h(\bx;\bW)} {\rm W}_{\rm ROT}(h(\bx_j;\bW),\hat{\by}_j)$ costs $O(Ld^2)$ by setting $l_j = 1$. Similar to the multi-label setting, using the decomposition (\ref{eqn:factorizeMahalanobis}), the cost reduces to $O(Lr^2)$. 

Overall, in both multi-class/multi-label settings, the cost of the gradient computation in (\ref{eqn:gradient_rot}) scales linearly with the number of labels $L$ and quadratically with $r$. When $r \ll d$, optimization of the ${\rm W}_{\rm ROT}$ loss becomes computationally feasible for large-scale multi-class/multi-label instances.






\section{Experiments}\label{sec:experiments}
We evaluate the proposed robust optimal transport formulations in the supervised multi-class/multi-label setting discussed in Section~\ref{sec:ROTloss}. Our code is available at \url{https://github.com/satyadevntv/ROT4C}. 



\begin{figure}[t]
\center
\includegraphics[width=.6\textwidth]{figs/mAP_v_epoch.pdf}
\caption{Evolution of mean average precision (mAP) on the Flickr tag-prediction dataset for various OT distance-based loss functions.}\label{fig:flickr}
\end{figure}





\subsection{Datasets and evaluation setup}
We experiment on the following three multi-class/multi-label datasets. 

\textbf{Animals} \citep{lampert13a}: This dataset contains $30\,475$ images of $50$ different animals. DeCAF features ($4096$ dimensions) of each image are available at \url{https://github.com/jindongwang/transferlearning/blob/master/data/dataset.md}. We randomly sample $10$ samples per class for training and the rest are used for evaluation.




\textbf{MNIST}: The MNIST handwritten digit dataset consists of images of digits $\{0,\ldots,9\}$. The images are of $28\times 28$ pixels, leading to $784$ features. The pixel values are normalized by dividing each dimension with $255$. We randomly sample $100$ images per class (digit) for training and $1000$ images per class for evaluation.

\textbf{Flickr} \citep{thomee16a}: The Yahoo/Flickr Creative Commons 100M dataset  consists of descriptive tags for around 100M images. We follow the experimental protocol in \citep{frogner15a} for the tag-prediction (multi-label) problem on $1000$ descriptive tags. The training and test sets consist of $10\,000$ randomly selected images associated with these tags. The features for images are extracted using MatConvNet \citep{vedaldi15a}. The train/test sets as well as the image features are available at \url{http://cbcl.mit.edu/wasserstein}. 

As described in Section~\ref{sec:ROTloss}, we use the fastText word embeddings \citep{bojanowski16a} corresponding to the labels for computing the OT ground metric in all our evaluations. 

We report the standard AUC metric for all the experiments. For the Flickr tag-prediction problem, we additionally report the mAP (mean average precision) metric. As the datasets are high dimensional, we use the low-dimensional decomposition of the Mahalanobis metric $\bM$ (Section~\ref{sec:low_dimensional_metric_decomposition}) for the proposed robust OT distance-based loss functions by randomly grouping the features. We experiment with $r\in\{5,10,20\}$. As baseline, we report the results with the ${\rm W}_2^2$ distance-based loss function (\ref{eqn:W22distance}) on all the datasets. Additional experimental details and results are in Section \ref{supp:sec:experiments}.



\begin{figure}[t]
\center
\includegraphics[width=.6\textwidth]{figs/flickr_timings.pdf}
\caption{Time taken per epoch versus $r$ on the Flickr dataset by our algorithm with the proposed ${\rm W}_{\rm P}$ loss with $k=1$.}\label{fig:timing}
\end{figure}






\subsection{Results and discussion}

We report the results of our experiments in Table~\ref{table:results}. Overall, the robust OT loss functions provide better generalization performance than the $\bW_2^2$ distance-based loss function. The proposed ${\rm W}_{\rm P}$ loss with $k=1$ obtains the best results on all the three datasets. The proposed ${\rm W}_{\rm P}$ loss with $k=2$ obtains a good AUC/mAP on the Animals and the Flickr datasets but does not generalize well in MNIST. Similarly, while ${\rm W}_{\rm DS}$ with $r=5$ obtains good results, its performance decreases with $r$. This is because the non-linear nature of the proposed OT distance-based loss function may lead to overfitting, especially at high $r$.

We also report the time taken per epoch of the SGD algorithm on the Flickr dataset with ${\rm W}_{\rm P}$ $(k=1)$ as the loss function. Our experiments are run on a machine with 32 core Intel CPU ($2.1$ GHz Xeon) and a single NVIDIA GeForce RTX 2080 Ti GPU ($11$ GB). The model computations are performed on the GPU. From Figure~\ref{fig:timing}, we observe that our model scales gracefully as $O(r^2)$ as discussed in Section~\ref{sec:algorithms}. Empirically, we show that we can obtain a good generalization performance and computational efficiency with $r\ll d$. 

\section{Conclusion}
We have discussed robust optimal transport problems arising from Mahalanobis parameterized cost functions. A particular focus was on discussing novel formulations that are less computationally heavy from an optimization viewpoint. We also proposed a  low-dimensional decomposition of the Mahalanobis metric for efficient computation of robust OT distances for high-dimensional data. 
%The parameter $r$ here allows to trade-off accuracy with computational benefit. 
An immediate result was that it allowed the use the robust OT formulations in high-dimensional multi-class/multi-label problems. Our experiments on real-world datasets suggest good performance of the robust OT loss in learning problems.




\section*{Acknowledgment}
We thank J. Saketha Nath for insightful discussions on the topic. 



